Locally tabular products of modal logics

In the product $L_1\times L_2$ of two Kripke complete consistent logics, local tabularity of $L_1$ and $L_2$ is necessary for local tabularity of $L_1\times L_2$. However, it is not sufficient: the product of two locally tabular logics may not be locally tabular. We provide extra semantic and axiomatic conditions that give criteria of local tabularity of the product of two locally tabular logics, and apply them to identify new families of locally tabular products. We show that the product of two locally tabular logics may lack the product finite model property. We give an axiomatic criterion of local tabularity for all extensions of $S4.1 [ 2 ]\times S5$. Finally, we describe a new prelocally tabular extension of $S{4}\times S{5}$.

==> above-s5-square.tex <==
%The proof given in \cite{NickS5} was algebraic.  
For a Kripke complete proper extension $L$ of $\LS{5}^2$, local tabularity can be obtained as a simple corollary of  
Theorem \ref{thm:criterion-frames-general} and observations in  Section \ref{subs:Prod}. Indeed, let $\clF$ 
be the class of point-generated frames of $L$.
By Lemma~\ref{lem:p-morph-sim}, $L \subseteq \Log{\quotfr{\clF}}$.  
So $\Log{\quotfr{\clF}}$ is a proper extension of $\LS{5}^2$ as well, and hence \(n = \sup\{m  \mid \exists F\in\clF\  \,(\quotfr{F}\toto \rect{m}{m} )\}\) is finite. 
For \(i = 1,\,2\), let $\clG_i$  
be the class of frames of form $\rect{X_1}{X_2}$ with $|X_i|\leq n$. 
By Lemma~\ref{lem:s5-square-quotient}, 
each frame in  $\quotfr{\clF}$ is isomorphic to a frame in $\clG_1 \cup \clG_2$. 
   Both classes $\clG_i$ are uniformly tunable by Theorem~\ref{thm:criterion-frames-general},
   and so is the class $\quotfr{\clF}$.\footnote{This is a particular case of the following general fact. 
   If the varieties generated by classes $\clC_1$ and $\clC_2$ are locally finite, then the 
   variety generated by  the class  $\clC_1 \cup \clC_2$ is locally finite as well:  $\clC_1 \cup \clC_2$ is uniformly locally finite by Malcev criterion 
   given in Theorem \ref{Malcev73}.}   
   %\cite[Section 14, Theorem 3]{Malcev73}.} 
   Then $L$ is locally tabular by Lemma~\ref{lem:quotient-uniformly-tunable}.


\hide{
 

\begin{lemma}\label{lem:ext-s5sq-complete}
Let $\clH$ be a class of bimodal frames such that $\Log\clH$ is a proper 
extension of $\LS{5}^2$. Then $\clH$
is uniformly tunable.
\end{lemma}
\begin{proof}
  Let \(\clF\) be the class of point-generated subframes of frames in $\clH$, and define  \(n = \sup\{m  \mid \exists F\in\clF\  \,(\quotfr{F}\toto \rect{m}{m} )\}.\) 
  Then \(n < \omega\) since otherwise \(\Log{\quotfr{\clF}} \subseteq\Log\{\rect{m}{m}\mid m < \omega\} = \LS{5}^2,\) and by Lemma~\ref{lem:p-morph-sim} \(L \subseteq \Log{\quotfr{\clF}} \subseteq \LS{5}^2.\) \ISH{That was difficult to follow. What is $L$?} By Lemma~\ref{lem:s5-square-quotient}, \(\quotfr{\clF} \subseteq \clF_1 \cup \clF_2,\)
   where \(\clF_i=\{\rect{k_1}{k_2}\mid k_1,\,k_2 < \omega,\, k_i \le n\}\) for \(i = 1,\,2.\) \ISH{I think it is wrong; one of cardinalities can be infinite}  
   Both classes $\clF_i$ are uniformly tunable by Theorem~\ref{thm:criterion-frames-general},
   and so is the class $\quotfr{\clF}$.\footnote{This is a particular case of the following general fact: 
   if the varieties generated by classes $\clC_1$ and $\clC_2$ are locally finite, then the 
   variety generated by  the class  $\clC_1 \cup \clC_2$ is locally finite as well. This fact is immediate from 
   \cite[Section 14, Theorem 3]{Malcev73}.} Then \(\Log{\clF}\) is locally tabular by Lemma~\ref{lem:quotient-uniformly-tunable}.
   \hide{
   The classes $\clF_i$ have the bounded cluster property, so their logics are locally tabular by Theorem~\ref{thm:criterion-frames-general}. Since \(\quotfr{\clF} \subseteq \clF_1 \cup \clF_2\), \(\Log \quotfr{\clF} \supseteq \Log \clF_1\cap \Log \clF_2\) is locally tabular. Then \(\Log{F}\) is locally tabular by Lemma~\ref{lem:quotient-uniformly-tunable}.
   }
\end{proof}

}

==> axiomatic-version.tex <==

\subsection{Axiomatic version}

Add subframe formula $S$ of a finite  cluster to one of the logics.
See \cite{CZ} for the transitive case.
An analog $S^*$ of the formula exists for a pretransitive case (immediate proposition).

\begin{proposition}\label{prop:adding-BCaxiom}
Let $L$ be a pretransitive logic of finite height. Then $L+S^*$ is locally tabular, whenever it is Kripke complete.
\end{proposition}
\begin{proof}
 Follows from the cluster criterion from \cite{LocalTab16AiML}.
\end{proof}


\begin{question}
Is $S^*$ canonical? Finitely canonical?

At least, let $L$ be a pretransitive logic of finite height. Is $L+S^*$ Kripke complete?
\end{question}


If yes, Kripke completeness in Proposition \ref{prop:adding-BCaxiom} is redundant.
Also,
this would give some axiomatic version of Theorem \ref{thm:criterion0}
and also some results for local tabularity of commutators $[L_1,L_2]$ (fusion + two commutativities +
Church-Rosser).
Notice that pretransitivity, finite height, and axioms of commutator are canonical.  Also, every locally tabular logic is finitely canonical, which is enough for Kripke completeness.

\begin{question}
Axiomatic version(s) of Theorem \ref{thm:criterion0};
axiomatic conditions when commutators $[L_1, L_2]$ are LT.
\end{question}



==> canonical-frame-lemma.tex <==
% For \(1\le m < \omega,\) define a formula
% \[
%   BCl_m = \Box_1\left(\bigvee_{i=0}^m \Box_2 p_i\right)\land \Box_2\left(\bigvee_{j=0}^n \Box_1 q_j\right) \to \bigvee_{i\ne i'}\Di_1 \Box_2 (p_i \land p_{i'}) \lor \bigvee_{j \ne j'} \Di_2\Box_1 (q_j\land q_{j'}).
% \]
% \begin{proposition}
%   Let \(F\models \LS{5}^2.\) Then \(F \models BCl_m\) if and only if for any point-generated subframe \((X,\,R_1,\,R_2)\) of \(F,\) either \(\left|\faktor{X}{R_1}\right|\le m\) or \(\left|\faktor{X}{R_2}\right|\le m.\)
% \end{proposition}

% Observe that \(BCl_m \not\in \LS{5}^2\) for any \(m\) since \(\mathbf{(m+1)}\times\mathbf{(m+1)}\not\models BCl_m.\)




This does not give a complete proof of Theorem \ref{thm:S5Nick}: we need to exclude the case of incomplete logics. 
For a logic $L$, let $F_L$ be its canonical frame \cite[Section 4.2]{BDV}. 
The following reasoning is a variant of the proof given in 
\cite[Claim 4.7]{NickS5};\footnote{We are grateful for an anonymous reviewer for providing the reference to this claim.} we provide it for the self-containment of the text. 
Together with the previous reasoning, it completes the proof of Theorem \ref{thm:S5Nick}.  
\begin{lemma}\cite{NickS5}\label{lem:ext-s5sq-canon}
If  $L$ is a proper extension of $\LS{5}^2$, then so is $\Log{F_L}$.
\end{lemma}
\begin{proof}%[Proof 1]
For the sake of contradiction, assume that \(\Log{F_L} = \LS{5}^2\). We show that in this case $L=\LS{5}^2$. 


Let $m<\omega$. By Proposition \ref{prop:Jankov-Fine}, %\ISH{Jankov-Fine for pretransitive frames}
$f:F\toto \rect{m}{m}$ for a point-generated subframe $F=(X,R_1,R_2)$ of $F_L$ and a p-morphism $f$. 


The logic $\LS{5}^2$ is canonical \cite{Segerberg2DimML}, \cite{Sheht-TwoDim78}.
It follows that $R_1$ and $R_2$ are equivalences, and for all $a,b\in X$, we have 
\begin{equation}\label{eq:cone}
a (R_1\circ R_2) b \text{ and } a (R_2\circ R_1) b.  
\end{equation}

For $i<m$, choose $d_i\in f^{-1}(i,i)$. 
For distinct $i,j<m$, we have
%\begin{equation}
  $(d_j,d_i)\notin R_1\cup R_2;$
%\end{equation}
hence, there is a formula $\delta_{ij}\in d_i$ such that 
$\Di_1\delta_{ij}\vee \Di_2\delta_{ij}\notin  d_j$. 
For $i>0$, put $\delta_i=\bigwedge_{i\neq  j<m} \delta_{ij}$; 
put $\delta_0=\bigwedge_{0<k<m} \neg (\Di_1\delta_{k}\vee \Di_2\delta_{k})$. 
We claim that
\begin{equation}\label{eq:dij}
\delta_i\in d_i.  
\end{equation}
For $i>0$, this is trivial. To show that $\delta_0\in d_0$, assume that 
$\delta_{k}\in a$ for some $a\in X$ and $k>0$.  Then 
$\delta_{k0}\in a$ and $\neg (\Di_1\delta_{k0}\vee \Di_2\delta_{k0})\in d_0$. 
Hence, $(d_0,a)\notin R_1\cup R_2$. Hence, $\neg (\Di_1\delta_{k}\vee \Di_2\delta_{k})\in d_0$.  


Define {\em horizontal} and {\em vertical}  sets: $H_i=\{a\in X\mid \Di_1 \delta_i\in a\}$,
$V_i=\{a\in X\mid \Di_2 \delta_i\in a\}$. 
We have
\begin{equation}\label{eq:lift}
R_1(d_i) \subseteq H_i \text{ and }R_2(d_i) \subseteq V_i. 
\end{equation}
Since $R_1$ and $R_2$ are equivalence relations, we also have 
%\VS{Looks like we need symmetry for \(R_1(H_i) \subseteq H_i\). Are we implicitly using the \(\LS{5}^2\)-consistency?}
\begin{equation}\label{eq:HVmon}
\text{$R_1[H_i]=H_i$ and $R_2[V_i]=V_i$.}
\end{equation}
All sets $H_i$ and $V_i$ are non-empty, since $d_i\in H_i\cap V_i$. 

Let us check that 
%\begin{equation}\label{eq:cover}
$\bigcup_{i<m} H_i=\bigcup_{i<m} V_i=X$.
%\end{equation}
For this, assume that $a\in X$, and $a\notin \bigcup_{0<i<m} V_i$. 
By \eqref{eq:cone}, $d_0R_1bR_2a$ for some $b$. Let $0<k<m$. 
Hence: $\neg \Di_1\delta_{k}\in b$, since $d_0 R_1b$; $\neg \Di_2\delta_{k}\in b$, 
since $bR_2a$; hence, $\delta_0\in b$, and so $a\in H_0$. Likewise, $\bigcup_{i<m} H_i=X$.

Let us check that  
%\begin{equation}\label{eq:disj1}
$H_i \cap H_j =\emp =V_i \cap V_j$ for distinct $i,j$. 
%$\end{equation} 
 Indeed, if $a\in H_i \cap H_j$, then $\Di_1 \delta_i\con \Di_1 \delta_j\in a$, and so $\delta_i\con \Di_1 \delta_j\in b$ for some $b\in R_1(a)$, which implies $i=j$.  Similarly for vertical sets.
It follows that $\{H_i\}_{i<m}$ and $\{V_i\}_{i<m}$ are $m$-element partitions of $X$.  
 

Put $C_{ij}=V_i \cap H_j$.  
%These sets are pairwise disjoint by \eqref{eq:HiVi}. 
By \eqref{eq:cone}, we have $d_i R_2 a R_1 d_j$ for some $a$, and so each $C_{ij}$ is non-empty
according to \eqref{eq:lift}. It follows that $\{C_{ij}\}_{i,j<m}$ is an $m^2$-element partition of $X$.
For $a\in C_{ij}$, put $g(a)=(i,j)$. 
Hence, $g$ maps $X$ onto $m\times m$. 

We claim that $g$ is a p-morphism. 
By \eqref{eq:HVmon}, $g$ is a homomorphism. 
It remains to check the back property. 
Let $a\in C_{ij}$, and assume that in $\rect{m}{m}$, $\tau$ is related to $(i,j)$
by the horizontal  relation. Then $\tau=(k,j)$ for some
$k<m$.
%\VS{Something wrong, is \(k\) just any?}
We have $a R_1 b R_2 d_{k}$ for some $b$ due to \eqref{eq:lift}. Hence, $b\in C_{kj}$ and so $g(b)=(k,j)$.  
The proof for $R_2$ is completely  analogous. 

Assume that a formula $\vf$ is satisfiable in a model $(\rect{m}{m},\theta)$. 
Define the following valuation $\eta$ on $F$: put
$\eta(p)=\bigcup\{C_{ij}\mid (i,j)\in \theta(p)\}$. 
Then $g$ is a p-morphism of $(F,\eta)$ onto $(\rect{m}{m},\theta)$. 
So $\vf$ is satisfiable in $(F,\eta)$. 

We have $(F,\theta_L)\mo L$, where $\theta_L$ is the restriction of the canonical valuation on $F$.  
Let $\psi_p$ be the formula $\bigvee \{\Di_1 \delta_i\con \Di_2 \delta_j \mid (i,j)\in \theta(p) \}$. 
For each $a\in X$, we have $a\in \eta(p) \text{ iff } \psi_p \in a,$
so $(F,\eta)\mo L$. It follows that $L=\LS{5}^2$. 
\end{proof}

\hide{
\begin{proof}
  By contraposition, assume that \(\Log{F_L} = \LS{5}^2.\)

  % Since \(\LS{5}^2 = \Log\{\rect{m}{m}\mid m < \omega\},\) there exist a number \(m < \omega,\) a valuation \(V\) of \(\rect{m}{m}\) and a point \(y\in m\times m\) such that \(\rect{m}{m},\,V,\,y\models \varphi.\)

  % Since \(\Log{F_L} = \LS{5}^2,\,F_L\not\models BCl_m,\) so there exists a point generated subframe \(C=(X,\,R_1,\,R_2)\) of \(F_L\) such that \(\left|\faktor{X}{R_1}\right|>m\) and \(\left|\faktor{X}{R_2}\right|>m.\) Then \(\rect{m}{m}\) is a p-morphic image of \(C.\)

  Fix \(m > 1.\) Let \(\chi_m\) be the Jankov-Fine formula of \(\rect{m}{m}, \) which is the conjunction of the following formulas:
  \begin{enumerate}
     \item \( p_{0,0};\)
     \item \(\bigwedge_{i,\,j<m} \Di_1 \Di_2 p_{i,j};\)
     \item \(\Box_1 \Box_2 \bigvee_{i,\,j < m}p_{i,j};\)
     \item \(\Box_1 \Box_2 \bigwedge_{i,j,j' < m}\left(p_{i,j} \to \Di_1 p_{i,j'}\right);\)
     \item \(\Box_1 \Box_2 \bigwedge_{i,j,j' < m}\bigwedge_{i'\ne i} \left(p_{i,j} \to \lnot\Di_1 p_{i',j'}\right);\)
     \item \(\Box_1 \Box_2 \bigwedge_{i,i',j < m}\left(p_{i,j} \to \Di_2 p_{i',j}\right);\)
     \item \(\Box_1 \Box_2 \bigwedge_{i,i',j < m}\bigwedge_{j'\ne j} \left(p_{i,j} \to \lnot \Di_2 p_{i',j'}\right).\)
   \end{enumerate}
   Since \(\Log{F_L} = \LS{5}^2,\) \(\chi_m\) is satisfiable in \(F_L:\) there exist a valuation \(V_m\) of \(C\) and a point \(c\in \dom F_L\) such that \(F_L,\,V_m,\,c\models V_m.\) Let \(C = F_L \uparrow x\) be the subframe generated by \(c.\)

   Pick representatives \(x_{i,j}\in V(p_{i,j})\) for \(i,\,j< m.\) Then the restriction of \(R_1,\,R_2\) on \(\{x_{i,j}\}_{i,\,j<m}\) forms a frame isomorphic to \(\rect{m}{m}:\)
   \begin{itemize}
     \item Since \(c\models \Box_1 \Box_2 \bigwedge_{i,j,j' < m}\left(p_{i,j} \to \Di_1 p_{i,j'}\right),\,\) and \(x_{i,j}\models p_{i,j},\) it is true \ISH{I do not see why} that \(x_{i,j} R_1 x_{i,j'}\) for any \(i,\,j,\,j'.\) Therefore \(R(x_{i,j}) \supseteq \{x_{i,j'}\}_{j'<m}.\)
     \item Since \(c\models\Box_1 \Box_2 \bigwedge_{i,j,j' < m}\bigwedge_{i'\ne i} \left(p_{i,j} \to \lnot\Di_1 p_{i',j'}\right),\) the negation of \(\Di_1 p_{i',j'}\) is true in \(x_{i,j}\) for any \(i'\ne i\) and any \(j'.\) Then \(R_1(x_{i,j}) \subseteq \{x_{i,j'}\}_{j'<m}.\) Therefore \(R_1(x_{i,j}) = \{x_{i,j'}\}_{j'<m}.\)
     \item Analogously, \(R_2(x_{i,j}) = \{x_{i',j}\}_{i' < m}\) for any \(i,\,j<m.\)
   \end{itemize}

   Find formulas \(\alpha_{i,j}\) that distinguish \(x_{i,\,j}\) as maximal \(L\)-consistent sets:
   \[
     V_L\uparrow C(\alpha_{i',j'})\cap \{x_{i,j}\}_{i,\,j<m} = \{x_{i',j'}\},\quad i',\,j'< m.
   \]
   Note that \(V_L\uparrow C\) is the restriction of the canonical valuation to \(C\), which is different from the valuation \(V_m\uparrow C\) which satisfies \(\chi_m.\)

   Since \(x_{i',j'}\not\in  R_1 (x_{i,j})\) for \(i'\ne i,\) there exists a formula \(\gamma_{i,j,i',j'}\in x_{i',j'}\) such that \(\Di_1 \gamma_{i,j,i',j'}\not \in x_{ij}.\) Analogously, for any \(i,\,j,\,i',\,j'\) with \(j\ne j',\) there is a formula \(\delta_{i,j,i',j'}\in x_{i',j'}\) such that \(\Di_2 \delta_{i,j,i',j'}\not \in x_{i,j}.\)

   For any \(i,\,j < m\) let
   \[
     \Phi_{i,j} = \alpha_{i,j} \land \bigwedge_{(i',j')\ne(i,j)} (\gamma_{i,j,i',j'} \land \delta_{i,j,i',j'}).
   \]
   Then \(V_L(\Phi_{i,j})\cap \{x_{i,j}\}_{i,j < m} = \{x_{i,j}\}.\)

   For any \(i<m-1\)  define
   \begin{gather*}
     \Psi_{i,j} = \Phi_{i,j}\land \bigwedge_{i'\ne i}\bigwedge_{j' < m} \lnot \Di_1 \Phi_{i',j'} \land \bigwedge_{i'<m} \bigwedge_{j'\ne j} \lnot \Di_2 \Phi_{i',j'} ,\quad j < m-1;\\
     \Psi_{i,m-1}= \Di_1 \Psi_{i,0}\land \bigwedge_{j<m-1} \lnot \Psi_{i,j}.
   \end{gather*}

   For \(i = m-1\) the formulas \(\Psi_{i,j}\) are defined differently:
   \begin{gather*}
    \Psi_{m-1,j} = \Di_2 \Psi_{0,j}\land \bigwedge_{i<m-1}\lnot \Psi_{i,j},\quad j < m-1;\\
    \Psi_{m-1,m-1} = \bigwedge_{i,j < m-1} \lnot \Psi_{i,j}\land \bigwedge_{i < m-1}\lnot \Di_1 \Psi_{i,0}\land \bigwedge_{j < m-1} \lnot \Di_2\Psi_{0,j}.
   \end{gather*}

   Let \(f:\:C \to m\times m\) be the map that sends every element of \(V_L\uparrow C(\Psi_{i,j})\) to \((i,j).\) To show that \(f\) is well-defined, we check that every \(x\in \dom C\) belongs to exactly one of \(V_L(\Psi_{i,j})\).

   Let \(x\in \dom C\) and assume \(x\not\in V_L (\Psi_{i,j})\) for any \(i,\,j<m-1.\) If \(\Psi_{i,0}\) is true at \(x\) for some \(i < m-1\) then \(x\in V_L(\Psi_{i,m-1});\) if \(\Psi_{0,j}\) is true at \(x\) for some \(j < m-1\) then \(x\in V_L(\Psi_{m-1,j});\) otherwise, \(x\in V_L(\Psi_{m-1,m-1}).\)

   Assume that \(C,\,V_L,\,x\models \Psi_{i,j}\land \Psi_{i',j'}\) for some \((i,\,j)\ne(i',j').\)
   \begin{itemize}
     \item If \(i = j = m-1\) then \(\Psi_{i',j'}\) is false in \(x\)
     \item If \(j = j' = m-1\) and  \(i,i' < m-1\) then
     \[
       C,\,V_L,\,x\models \Di_1 \Psi_{i,0} \land \Di_1 \Psi_{i',0};
     \]
     note that \(\Psi_{i,0}\) implies \(\lnot \Di_1 \Phi_{i',0}\) and \(\Psi_{i',0}\) implies \(\Di_1 \Phi_{i',0}.\) Then
     \begin{gather*}
        C,\,V_L,\,x\models \Di_1 \lnot \Di_1 \Phi_{i',0} \land \Di_1 \Di_1 \Psi_{i',0}\\
        C,\,V_L,\,x\models \Di_1 \Box_1 \lnot \Phi_{i',0} \land \Di_1 \Psi_{i',0},\\
      \end{gather*}
      so \(R_1(x)\) contains a point \(y\in V_L(\Psi_{i',0})\) and a point \(z\) such that \(R_1(z) \cap V_L(\Psi_{i',0}) = \varnothing.\) But \(R_1\) is an equivalence relation, so \(R_1(x) = R_1(z),\) a contradiction.
      \item Analogously, the case \(i = i' = m-1\) and \(j,\,j' < m-1\) leads to a contradiction since \(R_2\) is an equivalence relation.
     \item Finally, if \(i,\,j,\,i',\,j' < m-1\) then \(\Psi_{i,j}\) implies \(\Phi_{i,j}\) and hence \(\Di_1 \Phi_{i,j}\) by the reflexivity of \(R_1;\) \(\Psi_{i',j'}\) implies \(\lnot \Di_1 \Phi_{i,j},\) a contradiction.
   \end{itemize}

   Then \(f\) is well-defined.

   Let \(V\) be any valuation on \(\rect{m}{m}.\) We construct a new valuation \(V^*\) on \(C\) by setting
   \[
     V^*(p) = \bigcup \{V_L\uparrow C(\Psi_{i,j}) \mid (i,\,j)\in V(p)\}.
   \]
   We claim that \(f\) is a p-morphism of models from \((C,\,V^*)\) to \((\rect{m}{m},\,V).\)

   By the construction,
   \begin{align*}
     f(x)\in V(p) &\iff \exists (i,j):\:f(x) = (i,j)\text{ and }(i,j)\in V(p)\\
     &\iff \exists (i,j):\:x\in V_L\uparrow C(\Psi_{i,j}) \text{ and }(i,j)\in V(p)\\
     &\iff x\in \bigcup \{V_L\uparrow C(\Psi_{i,j}) \mid (i,j)\in V(p)\}\iff x\in V^* (p).
   \end{align*}

   Let \(x,\,y\in \dom C\) and \(x R_1 y.\) Find \(i,\,j\) such that \(x\in V_L(\Psi_{i,j})\) and \(i',\,j'\) such that \(y\in V_L(\Psi_{i',j'}).\) If \((i,\,j)=(i',\,j')\) then \(f(x) = f(y),\) hence \(f(x) R_1 f(y)\)   by reflexivity of \(\rect{m}{m}.\) Then assume \(j\ne j'\) and show that \(i = i'.\) Since \(xR_1 y,\,\) \(x\in V_L( \Psi_{i,j}\land \Di_1 \Psi_{i',j'}).\) If \(i,\,j,\,i',\,j' < m-1\) then \(x\models \lnot \Di_1 \Phi_{i'',j'}\)  for any \(i''\ne i.\) But \(\Di_1 \Psi_{i',j'}\) entails \(\Di_1 \Phi_{i,j},\) so it's only possible that \(i = i'.\) If \(i = m-1\ldots?\)

   % Show that \(R_1\cap R_2(x_{i,j}) = V_L(\Psi_{i,j})\) for \(i,\,j < m-1.\)
   % \begin{description}
   %   \item[\((\subseteq)\)] If \(i'\ne i,\,i'<m-1\) then \(\Psi_{i',j}\) implies \(\lnot \Di_1 \Phi_{i,j}.\) Since \(x_{i,j}\in V_L(\Phi_{i,h}),\) it follows that \(R_1(x_{i,j})\) does not contain points from \(V_L(\Psi_{i',j})\) for \(i'<m-1. \) Analogously, \(R_2(x_{i,j})\) does not contain points from \(V_L(\Psi_{i,j'})\) for \(j' \ne j,\,j' < m-1.\) If
   %   \item[\((\supseteq)\)]
   % \end{description}


   Let \(f(x)=(i,j) R_1 (i',j').\) Then \(x\in V_L(\Psi_{i,j}).\)
\end{proof}
}


Now Theorem \ref{thm:S5Nick} follows: 
if $L$ is a proper extension of $\LS{5}^2$, then 
so is the logic 
$\Log F_{L}$ of the canonical frame of $L$; the latter logic is Kripke complete and so is locally tabular;
since $\Log F_{L}\subseteq L$, $L$ is locally tabular.

\hide{
\ISH{Obsolete:

This lemma reduces the question about LT extensions of $\LS{5}^2$ to the Kripke complete case.
Indeed, we have $\Log(F_{L})\subseteq L$, and the first one is LT according to the known semantic argument. } 
}

==> store_above_S4_2_2024-12-30.tex <==
\section{Products above $\LS{4}^2$ (old; sort it out)}




\subsection{Productivization}\label{subs:Prod}  
 \begin{definition}\label{def:tilde}
  Let \(F = (X,\,(R_\Di)_{\Di\in A})\) be an \(\AlA\)-frame, where all $R_\Di$ are preorders. Define the equivalence relation
  $
    {\sim}=\bigcap_{\Di\in A} (R_\Di\cap R_\Di\inv).
  $
  The quotient frame $\fact{F}{\sim}$ is denoted  \(\widetilde{F}\).   
  Given a class \(\clF\) of \(\AlA\)-frames, let %\(\quotfr{\clF}\) denote the class
  \(\quotfr{\clF} = \{\quotfr{F} \mid F\in \clF\}.\)
 \end{definition}
\ISH{Where to move? -  Note that if \(F=(X,R_1,R_2)\) is an \(\LS{5}^2\)-frame, then \({\sim}\) is $R_1\cap R_2$.}
   \hide{
  \(= (\fact{X}{\sim},\,(\quotfr{R_\Di})_{\Di\in\Al})\) the minimal filtration\ISH{do we need this term?} of \(F\) with respect to \(\sim:\)
  \[
    [a] \quotfr{R_{\Di}} [b] \iff \exists a'\in[a]\ \exists b'\in [b]\ \left(a' R_{\Di} b' \right),\quad \Di\in \AlA.
  \]
  }
  
\begin{lemma}\label{lem:p-morph-sim}
  If the relations of \(F\) are
  %transitive, 
  preorders,
  then \(F\toto \quotfr{F}.\)
\end{lemma}
\begin{proof}
For any frame, the quotient map is a surjective homomorphism. To check the back condition, assume that \([a]\quotfr{R_\Di}[b]\) for some \(a,\,b\in X\) and \(\Di\in \AlA.\) Then \(a' R_\Di b'\) for some \(a'\sim a\) and \(b'\sim b.\) By the definition, \(a  R_\Di a'\) and \(b' R_\Di b,\)  so \(a  R_\Di a' R_\Di b' R_\Di b ,\) hence \(a R_\Di b\) by transitivity.
\end{proof}

\begin{definition}\label{def:sum-over-frame}
Consider an $\Al$-frame $I=(Y,(S_\Di)_{\Di\in \Al})$
and a family $(F_i)_{i\in Y}$ of $\Al$-frames
$F_i=(X_i,(R_{i,\Di})_{\Di\in \Al})$.
The {\em sum
 $\LSum{I}{F_i}$ of the family $(F_i)_{i\in Y}$ over~$I$}
 is the $\Al$-frame $(\bigsqcup_{i \in Y} X_i, (R^\Sigma_\Di)_{\Di\in \Al})$,
 where
 $\bigsqcup_{i\in Y}{X_i}=\bigcup_{i\in Y}(\{i\}\times X_i)$,\extended{is the  disjoint union of sets $X_i$} and
$$(i,a)R^\Sigma_\Di (j,b) \quad \tiff \quad (i = j \text{ and }a R_{i,\Di} b) \text{ or } (i\neq j \text{ and } iS_\Di j).$$
For  classes $\clI$, $\clF$  of $\Al$-frames,
let $\LSum{\clI}{\clF}$  be the class of all sums
$\LSum{I}{F_i}$ such that $\frI \in \clI$ and  $F_i\in \clF$ for every $i$ in $\frI$.
\end{definition}
\begin{theorem}\cite{LTViaSums2022}\label{thm:sum}
Let $\clF$ and $\clI$ be classes of $\Al$-frames.
If the   logics $\Log{\clF}$ and
$\Log{\clI}$ are locally tabular, then  $\Log{\LSum{\clI}{\clF}}$  is locally tabular as well.
\end{theorem}

\begin{lemma}\label{lem:quotient-uniformly-tunable}
  Let \(\clF\) be a class of frames such that in every $F\in\clF$, all relations are 
  %transitive. 
  preorders.
  Then \(\Log\quotfr{\clF}\) is locally tabular iff \(\Log\clF\) is locally tabular.
\end{lemma}
\begin{proof}[Proof via sums]
  The `if' direction is trivial, since $\Log\clF\subseteq \Log\quotfr{\clF}$ by Lemma \ref{lem:p-morph-sim}.

  `Only if'.
  Consider \(F=(X,\,(R_\Di)_{\Di\in \AlA})\in \clF.\) Let \(\sim\) be defined as in Definition~\ref{def:tilde}, and denote \(Y = X/{\sim}.\)
  
  We claim that \(F \cong \LSum{\quotfr{F}}({F\restr U})\), where \(U\subseteq X\) ranges over the equivalence classes in \(Y\). Define \(f:\:X \to \bigsqcup_{U \in Y} U\) by \(f(a) = ([a]_{\sim},\,a).\) It is trivial that \(f\) is injective. If \((U,\,a)\in \bigsqcup_{U \in Y} U\) then \(a\in U\subseteq X\) by the definition, so \(U = [a]_{\sim},\) hence \((U,\,a) = f(a).\) Then \(f\) is surjective.

  Suppose \(a,b\in X,\,a R_\Di b.\) If \(a \sim b\) then \(f(b) = ([a]_{\sim},\,b),\) so \(f(a)R^\Sigma_\Di f(b).\) Otherwise~\([a]_{\sim} {\ne} [b]_{\sim};\) observe that \([a]_{\sim} \quotfr{R_\Di} [b]_{\sim}\) by the definition of \(\quotfr{R_\Di},\) so~\(f(a) R^\Sigma_\Di f(b).\) 

  Conversely, let \(f(a) R^\Sigma_\Di f(b).\) If \([a]_{\sim} {=} [b]_{\sim}\) then \(a R_\Di b;\) if \([a]_{\sim}{\ne} [b]_\sim\) then \([a]_\sim \quotfr{R_\Di} [b]_\sim.\) By the definition of~\(\quotfr{R_\Di},\) there exist \(a'\sim a\) and \(b'\sim b\) such that \(a' R_\Di b'.\) By the definition of \(\sim,\) \(a R_\Di a'\) and \(b' R_\Di b,\) so by transitivity \(a R_\Di b.\) 

  The isomorphism implies that \(\Log\clF = \Log{\LSum{\quotfr{\clF}}{\clG}}\) where \(\clG\) is the class of all frames~\(F\restr U\) where \(F\in \clF\) and \(U \in \dom F/{\sim}.\)
  In any frame of \(\clG,\) the relations are transitive and symmetric by the definition of \(\sim\). Then \(\clG\) is uniformly tunable since on the frames of \(\clG\) any partition is tuned, so \(\Log \clG\) is locally tabular by Theorem~\ref{thm:LFviaTuned}. By hypothesis, \(\Log \quotfr{\clF}\) is also locally tabular. Then \(\Log\clF\) is locally tabular by Theorem~\ref{thm:sum}.
\end{proof}


\begin{proof}[Direct proof]
  The `if' direction is trivial, since $\Log\clF\subseteq \Log\quotfr{\clF}$ by Lemma \ref{lem:p-morph-sim}.

  `Only if'. 
   Assume that all frames in $\quotfr{\clF}$ are $f$-tunable.  
  Let \(\clV\) be a finite partition of $F$, $n=|\clV|$. 
Let \(\sim\) be defined as in Definition~\ref{def:tilde}. 
For $\sim$-classes $[x],[y]$, put $[x]\approx [y]$ iff 
$$
\AA V\in \clV \, ([x]\cap V\neq \emp   \tiff [y]\cap V\neq \emp )
$$
Readily, $\approx$ has at most $ 2^n$ equivalence classes. Let $\clU$ be the corresponding partition of $\quotfr{\clF}$. 
There is a tuned refinement $\clW$ of $\clU$ of size at most $f(2^n)$. 
Now put $x\equiv y$ iff ($x\sim_\clV y$ and $[x]\sim_\clW[y]$). 

It is straightforward that the quotient of $F$ by this equivalence 
is tuned, and its size does not exceed  $nf(2^n)$. 
\IS{Check the notation; check the details.} 
\end{proof}


\begin{lemma}\label{lem:s5-square-quotient}
  Let $F=(X,R_1,R_2)$ be a point-generated $\LS{5}^2$-frame,
  $|\fact{X}{R_1}|=\kappa$, $|\fact{X}{R_2}|=\mu$. 
  Then $\quotfr{F}$ is isomorphic to $\rect{\kappa}{\mu}$.
\end{lemma}
\IS{An important variation: 
Can we get prpp-criterion for the clusters in $\LS{4}\times \LS{4}$-frames? 

\hide{
Let $C$ be a cluster in an $\LS{4}\times \LS{4}$-frame, (AND SOMETHING ELSE)
$|\fact{C}{R_1}|=\kappa$, $|\fact{C}{R_2}|=\mu$. 
Then $\quotfr{C}$ is isomorphic to $\rect{\kappa}{\mu}$.

(We need to carefully check if there is an analog in earlier works.)
}
}

\begin{proof}
  Let \(\{H_\alpha\}_{\alpha < \kappa}\) and \(\{V_\beta\}_{\beta < \mu }\) be the elements of \(\fact{X}{R_1}\) and \(\fact{X}{R_2},\) respectively. We claim that \(H_\alpha\cap V_\beta\ne \varnothing\) for any \(\alpha< \kappa,\,\beta < \mu.\) Let \(a \in H_\alpha\) and \(b\in V_\beta.\) Since \(F\) is point-generated, \(b\in R_2[R_1(a)],\) so there exists \(c\in X\) such that \(a R_1 c\) and \(c R_2 b.\) Then \(c \in R_1(a) = H_\alpha\) and \(c\in R_2(b) = V_\beta,\) so \(c\in H_\alpha\cap V_\beta.\) 

  Define \(f:\:\kappa\times \mu \to \fact{X}{\sim}\) by \(f(\alpha,\,\beta) = H_\alpha \cap V_\beta.\) 
  We claim that \(f\) is an isomorphism between \(\rect{\kappa}{\mu}\) and \(\quotfr{F}.\) 
  For any \([a]\in \fact{X}{\sim}\) there exist unique \(H_\alpha,\,V_\beta\) such that \(a\in H_\alpha \cap V_\beta,\) so \([a] = H_\alpha\cap V_\beta,\) thus \(f\) is a bijection. 
  Let $R_H$ and $R_V$ denote the horizontal and vertical relations in \(\rect{\kappa}{\mu}\). If \((\alpha,\beta) R_H (\alpha',\beta')\) then \(\alpha = \alpha'.\) Consider \(a\in H_\alpha\cap V_\beta\) and \(b\in H_\alpha\cap V_\beta'.\) Observe that \(H_\alpha = R_1(a),\) so \(a R_1 b,\) thus \(f(\alpha,\beta) = [a] \quotfr{R_1}[b] = f(\alpha',\beta').\) Conversely, if \(f(\alpha,\beta) \quotfr{R_1} f(\alpha',\beta'),\) there exist \(a\in H_\alpha\cap V_\beta\) and \(b\in H_\alpha'\cap V_\beta'\) such that \(a R_1 b.\) Then \(H_\alpha = R_1(a) = R_1(b) = H_\alpha',\) so \(\alpha = \alpha'\) and \((\alpha,\beta) R_H (\alpha,\beta') = (\alpha',\beta').\) An analogous argument applies for \(R_V.\) %\ISH{$R_H$ and $R_V$ seem to be undefined}
\end{proof}

\extended{
\begin{proposition}\label{prop:rpp-factor}
Assume that in every frame in a class  $\clF$  of $\Al$-frames all relations are transitive. 
Then 
$\clF$ has rpp iff 
$\fact{\clF}{\sim}$ has the rpp. 
\end{proposition}
\begin{proof}
    \ISH{Seems to be trivial. DC, write down}
    \ISH{Seems to be obsolete; move to Store?}
\end{proof}
}

\subsection{Logics above $\LS{5}^2$}\label{subs:s5sq}

An important fact about $\LS{5}^2$ was established in \cite{NickS5}: this logic is {\em prelocally tabular}, that is the following theorem holds. 
\begin{theorem}\cite{NickS5}\label{thm:S5Nick}
All proper extensions of $\LS{5}^2$ are locally tabular.    
\end{theorem}
 

\input{above-s5-square}


\hide{

Idea: $L$ is Kripke-complete proper extension of $\LS{5}^2$. 
Then there is a pair of ``nice'' products logics.\\
$L \supseteq L_{complete}$ (known )\\ 
$\supseteq \Log(\text{sums over products})$  (general observation: local tabularity is preserved at this step; special observation: Lemma about $\LS{5}^2$) \\
$\supseteq$ (=?) intersection of two logics of products 


\ISH{Would it be simpler to proof the following argument?}
\begin{lemma}
Assume that $L$ is a Kripke complete proper extension of $\LS{5}^2$.  
Then $L\cap\ML(\Di_1)$ or $L\cap \ML(\Di_2)$ has the bounded cluster property.  

\ISH{Or, in terms of frames:}
Let $\clF$ be a class of $\LS{5}^2$-frames. If ...

\end{lemma}
}






\input{canonical-frame-lemma}

\subsection{The product of pretabular logics can be not prelocally tabular}


A logic is {\em tabular}, if it is characterized by a single finite frame. A 
non-tabular logic is {\em pretabular}, if all of its proper extensions are tabular. 
There are exactly five pretabular logics above $\LS{4}$, see \cite{EsakiaMeskhi1977}, \cite{MaksimovaPretab75}, or \cite[Section 12.2]{CZ}. One of them is the logic $\LS{5}$. 
Another is the logic $\TL$ defined below. 
While $\LS{5}^2$ is prelocally tabular,
%\VS{define}, 
it turns out that products of pretabular logics can be not prelocally tabular. 



The {\em tack frame} $\TF$ is the ordered sum $(\omega+1,R)$ of a countable cluster and a singleton, that is
$\alpha R \beta$ iff $\alpha<\omega$ or $\beta=\omega$. 
Let $\TL$ be the logic of its frame.% $\TL$ is one of exactly five pretabular (that is, characterized by a single finite frame) logics above $\LS{4}$.

In this subsection we show that $\TL\times \LS{5}$ is not prelocally tabular, and give an axiomatic criterion of local tabularity of its extensions.  

 

\begin{proposition}
$\TL\times \LS{5}$ is not prelocally tabular. 
\end{proposition}
\begin{proof}
%Consider the frame $H=(2,\leq)\times\mathbf{2}$. 
%Readily, 
%$H$ validates $\TACK\times \LS{5}$. 
Let $H=T\times \boldsymbol{\omega}$. 
The formula 
$\vf=\Di_2\Di_1\Box_1 p\imp \Box_1\Di_1 p$ is not valid in $H$: consider a model
$M=(H,\theta)$ with $\theta(p)=\{(\omega,1)\}$; then $\vf$ is falsified in $M$ at $(0,0)$.

Consider the equivalence $\equiv$ on $\dom H$ that extends the diagonal 
by the set of pairs of form $((\omega,m),(\omega,n))$.\improve{ \ISH{Clumsy}}
It is easy to check \ISH{DC} that $H  \toto \fact{H}{\equiv}$, 
hence the logic $L$ of the latter frame extends $\TL$. 
It is also straightforward that $\vf$ is valid in $\fact{H}{\equiv}$, so $L$ is a proper extension of $\TL$. Finally, we observe that $L$ is not locally tabular:  
$\fact{H}{\equiv}$ contains $\rect{\omega}{\omega}$ as a subframe, and the logic $\LS{5}^2$ of this subframe is not locally tabular. 
\end{proof}


\newpage 


% We say that a bimodal frame $(X,R,E)$ is {\em simple}, \IS{Let us keep old notation: $(X,R,\approx)$ }
% if $E=X\times X$. 
A point \(a\in X\) is called \emph{\(R\)-maximal}
\IS{I suggest: $R$-terminal} in a transitive frame \((X,R)\), if \(R(a) = \{a\}\).
\begin{lemma}\label{lem:S4.1[h]xS5_simple}
    Let \(C = (X, R, E)\in \clusters{\LS{4.1}[h]\times \LS5}\) be a cluster that contains an \(R\)-maximal element, where \(h < \omega\).
    Then~\(C\) is simple.
\end{lemma}
\begin{proof}
    If \(X\) is empty, then the statement is trivial, so we will assume \(X \ne \emp.\)
    We say that a point \(a\in X\) is \emph{quasiminimal}, if \(R\inv(a) \subseteq R(a)\).
    Let~\(Y\) be the set of quasiminimal points in~\(C.\)
    An induction on~\(h\) shows that \(Y\ne \emp\).
    By the definition of~\(Y\) and the reflexivity of~\(R\) we have \(R\inv[Y] = Y.\)
    
    Let \(Z\) be the set of \(R\)-maximal points. By the assumption, \(Z\ne \emp\).
    For any \(a\in Z\) and \(b\in Y\), we have \(b\in E[R(a)] = E(a)\).
    Then \(Z \cup Y\) is contained in an~\(E\)-equivalence class.

    Now let \(a\in X\).
    Since \(C\) has finite height, there exists \(b\in Y\) such that~\(b R a\). \VS{\emph{Do we need more details here?}}
    Since \(C\) is a cluster, there exists \(c\in X\) such that \(a E c R b.\)
    Then \(c\in R\inv[Y] = Y.\)
    Therefore \(a\) belongs to the \(E\)-equivalence class that contains \(Y.\)
    Since \(a\in X\) was arbitrary, it follows that \(X\) consists of one \(E\)-equivalence class.
\end{proof}

 Let~\(\clF_h\) be the class of all frames \((X,R,E)\models\LS{4.1}[h]\times \LS5\) such that~\(R \not\subseteq E.\)
  For any~\(F = (X,R,E)\in \clF_h,\) let~\(Q_F \subseteq \clusters{F}\) be the set of all clusters in~\(F\) that contain an~\(R\)-maximal element.
  We define \(\alpha(F)\) to be the subframe \(F \restr\left(W \setminus \bigcup Q_F\right).\)

  \begin{proposition}
    If \(F\in \clF_h\), then \(\alpha(F)\) is not empty.
  \end{proposition}
  \begin{proof}
      By contraposition.
      Let \(F=(X,R,E)\) and assume that~\(\alpha(F)\) is empty.
      Then \(X = \bigcup Q_F.\)
      Let \(a,\,b \in X\) be such that \(a R b.\)
      The cluster of \(a\) contains an \(R\)-maximal element \(c\), so~\(c E a\) by Lemma~\ref{lem:S4.1[h]xS5_simple}.
      Then \(b\in R[E(a)] = E[R(a)] = E(a)\).
      It follows that \(R \subseteq E,\) so \(F\not\in \clF_h.\)
  \end{proof} 

  \begin{proposition}
      For any \(F\in \clF_h,\) where \(h < \omega,\) the logic \(\LS{4}[h-1]\times\LS5\) is valid in \(\alpha(F)\).
  \end{proposition}
  \begin{proof}
      \todo{Need to discuss how to convey the following facts:
        \begin{itemize}
            \item \(\LS{4}[h] \times \LS5\) is product-matching
            \item \(\LS4\) and \(\LS5\) are subframe
        \end{itemize}
      }
  \end{proof}

  \begin{proposition}\label{prop:alpha_transfers_rpp}
     Let \(h < \omega.\)
     If \(F \subseteq \clF_h,\) then \(F\models \RP_m(1,1)\) iff~\(\alpha(F)\models \RP_{m-2}(1,1).\)
  \end{proposition}
  \begin{proof}
    The 'only if' direction holds since~\(\RP_m(1,1)\) is subframe. 
    
    To show the 'if' direction, let~\(\alpha(F)\models \RP_{m-2}(1,1).\)
    Let us consider a product path~\(a_0,\,\ldots,\,a_{m+1}\) in~\(F=(X,R,E).\)
    If~\(a_0,\,\ldots,\,a_{m-1}\not\in \bigcup Q_F,\) then by the product rpp for~\(\alpha(F)\) this path can be reduced to a product path of~\(m-1\) points. Then the path~\(a_0,\,\ldots,\,a_{m+1}\) can be reduced to a product path of at most \(m+1\) points.
    Otherwise, let~\(a_i\in \bigcup Q_F\) for some~\(i \le m-1\). Let~\(C\) denote the cluster of~\(a_i.\)
    Then~\(R(a_i) \subseteq C \subseteq E(a_i)\) by Lemma~\ref{lem:S4.1[h]xS5_simple} and \todo{Make it a separate proposition}.
    Then~\(a_j\in C\), and therefore \(a_i E a_j\), for all~\(i \le j \le m+1\).
    In particular,~\(a_{m-1} E a_m E a_{m+1}\).
    Then~\(a_0,\,\ldots,\,a_{m-1},\,a_{m+1}\) is a product path.
  \end{proof}

  \begin{proposition}\label{prop:alpha_transfers_lt}
    For any class of frames \(\clF \subseteq \clF_h,\) \(\Log \clF\) is locally tabular iff~\(\Log \alpha[\clF]\) is locally tabular.
  \end{proposition}
  \begin{proof}
    Both classes are of uniformly finite height, so we only need to show that~\(\clusters{\clF}\) is uniformly tunable iff~\(\clusters{\alpha[\clF]}\) is.
    Indeed, observe that~\(\clusters{\clF} = \clusters{\alpha[\clF]} \sqcup \bigcup \{Q_F \mid F\in \clF\}.\)
    By Lemma~\ref{lem:S4.1[h]xS5_simple}, \(\{Q_F \mid F\in \clF\}\) is uniformly tunable, since~\(\LS{4.1}[h]\) is locally tabular. \VS{\emph{Need more details?}}
  \end{proof}
 
We say that \emph{the product rpp criterion} holds for a logic \(L\), if for any normal extension \(L'\) of \(L,\) it is true that
\begin{center}
    $L'$ contains a product rpp formula iff  $L'$ is locally tabular. 
\end{center}

\begin{theorem}
    If the product rpp criterion holds for~\(\LS{4}[h]\times  \LS5\), then it also holds for~\(\LS{4.1}[h+1] \times  \LS5,\) for any \(h < \omega.\)
\end{theorem}
\begin{proof}
    Let~\(h < \omega\). Assuming the product rpp criterion for \(\LS{4[h]}\times  \LS5\), we will show it for~\(\LS{4.1[h+1]}\times \LS5.\)

    
    Let~\(L\) be a locally tabular normal extension of~\(\LS{4.1}[h+1]\times \LS5.\)
      Then~\(L\) has the product rpp by the \todo{decoloring argument}.
    
    
    Conversely, let~\(L\) be a normal extension of~\(\LS{4.1}[h+1]\times \LS5\) containing~\(\RP_m(1,1).\)
      Then~\(F_L \models \RP_m(1,1).\)
      By Proposition~\ref{prop:alpha_transfers_rpp},~\(\alpha(F_L) \models \RP_{m-2}(1,1).\)
      Then by the assumption~\(\Log \alpha(F_L)\) is locally tabular.
      By Proposition~\ref{prop:alpha_transfers_lt}, so is~\(\Log F_L \subseteq L.\)
      Then~\(L\) is locally tabular.
\end{proof}
\begin{corollary}
    The product rpp criterion holds for \(\LS{4.1}[2]\times \LS5.\)
\end{corollary}
\todo{Some words about \(\LS{4.1}[3]\times \LS5\)? A reference to Meadors?}
\IS{Yes, I think it would be nice if we announce his result. Let us include the reference. Something like this (wording is very preliminary): 
\begin{remark}
After the first version of this paper appeared online, 
it was announced in a recent manuscript \cite{...} that this criterion  generalizes for (h=2), 
, which implies (h=2+ .1).
\end{remark}
}

\newpage 
!!!\todo{OLD VERSION --- REMOVE IT LATER}
Let $\LS{4.1[2]}$ be the extension of $\LS{4}$ with the axioms  
$\Box\Di p\imp \Di \Box p$ and $B_2$.  
In transitive frames,  $\Box\Di p\imp \Di \Box p$ defines the first-order property
 %\cite{HandBookML}
\begin{equation}\label{eq:s4.1-condition}
  \forall x\,\exists y\,\left(xRy \land \forall z \left(yRz \to z = y\right)\right),
\end{equation}
see, e.g., \cite[Section 3.7]{BDV}.
The tack frame \(T\) has this property; since it is transitive and has height \(2,\) $\LS{4.1[2]}\subseteq \TL$\IS{Most probably, they are equal and this is known; perhaps, we can avoid this inclusion.}.

We say that a bimodal frame $(X,R,\approx)$ is {\em simple}, 
if $\approx$ is $X\times X$.
% \VS{Define the alphabet; should we write \((X,\,(R,\approx))\) with the relations in parentheses?} 
% \ISH{I think it is fine in this case; even formally: an ordered triple is a pair of ordered pairs.
% We can also use $(X;R,S)$, if something looks really confusing. }
\begin{lemma}\label{lem:tack-sim}
Every cluster in $\clusters{\LS{4}.1 [ 2 ] \times \LS{5}}$ 
  is a point-generated $\LS{5}^2$-frame, or a simple frame. 
%$\fact{C}{\sim}$ is a rectangle.
\end{lemma}
\begin{proof}
Let $C=(X,R,\approx) \in\clusters{\LS{4}.1 [ 2 ] \times \LS{5}}$.
The frame $(X,R)$ is a preorder and $\approx$ is an equivalence on $X$, and we have
 $R\,\circ\, \approx\; = \; X\times X$. 
 Assume that $C$ is not simple.  
 We claim that in this case $R$ is symmetric. Assume $xRy$. 
 There is $z\in X$ such that $y\not\approx z$. We have $yRz'\approx z$ for some $z'$.
 Then $y\neq z'$. It follows that $y$ is not maximal in $(X,R)$ since by \eqref{eq:s4.1-condition} the maximality would imply \(R(y) = \{y\}.\)
 \hide{\ISH{Details about $\Box\Di p \imp \Di\Box p$}\VS{Done}. \ISH{Fine!} }
 Hence $yRx$.
\end{proof}

We conclude this paper with the following axiomatic criterion of local tabularity above 
$\LS{4}.1 [ 2 ]\times \LS{5}$.
\begin{theorem}\label{thm:some-axiomatic-crit} Let $L$ be an extension of $\LS{4}.1 [ 2 ]\times \LS{5}$.
Then $L$ is locally tabular iff for some $m$, $L$ contains the  product rpp formula $\RP_m(1,1)$. 
\end{theorem} 
\begin{proof}
%The `only if' direction is given by  Corollary \ref{cor:criterion-logics-general}.
The `only if' direction 
follows from Theorem \ref{thm:ShSh:RP}  and Proposition \ref{prop:rpp-to-modal-poly}.
\ISH{We need more details here:   

Consider the {\em decoloring} translation $[\Di \vf]=\Di_a[\vf]\vee \Di_b[\vf]$ which respects Boolean connectives, and the  following unimodal  fragment $L_0$ of $L$: $\{\vf \mid [\vf]\in L\}$. Then $L_0$ is locally tabular. 
Now (with some more efforts) the `only if' direction 
follows from Theorem \ref{thm:ShSh:RP}  and Proposition \ref{prop:rpp-to-modal-poly}.
}

`If'. 
 Let $F_L$ be the canonical frame of $L$, 
$\clC$ the set of cluster frames in $F$, 
$\clC_0$ the set of simple frames in $\clC$, and $\clC_1$  the set of other frames in $\clC$. 

%Reviewer: "... in F, C_0 that of simple frames in C, and C_1 that of other frames in C.".

Since the logic $\LS{4}.1 [ 2 ]$ is locally tabular, the class of its frames is uniformly tunable, and so 
is $\clC_0$. 


%Let $F_L=(X,R_1,R_2)$. Since $R_1$ and $R_2$ are preorders, $(X,R_1\cup R_2)$ validated 
%, and so $F_L$ has the rpp. 
By Proposition \ref{prop:rpp-canon}, $F_L\mo \RP_m(1,1)$. 
Due to  the first order characterization of $\RP_m(1,1)$ given in Proposition \ref{prop:rpp-to-modal-poly}, $\RP_m(1,1)$ is valid in each subframe $C\in \clC_1$ of $F_L$.\improve{\ISH{Is it evident, or some proposition is required?}}  
Hence, we have  $\clC_1\mo \RP_m(1,1)$. 
By Lemma \ref{lem:tack-sim}, the logic $L_0$ of $\clC_1$ is an extension of $\LS{5}^2$; 
since $\RP_m(1,1)$ is not in $\LS{5}^2$, this extension is proper. 
By Theorem \ref{thm:S5Nick}, $L_0$ is locally tabular, and so  $\clC_1$
is uniformly tunable.  
\hide{
So 
$\quotfr{\clC_1}\mo\RP_m(1,1)$ by Lemma \ref{lem:p-morph-sim}. 
By Lemma \ref{lem:tack-sim}, $\clC_1$ consists of point generated $\LS{5}^2$-frames, and so  $\quotfr{\clC_1}$ consists of rectangles according to Lemma \ref{lem:s5-square-quotient}. 
By Corollary \ref{cor:criterion-logics-general}, \ISH{DOES NOT APPLY HERE} the logic of $\quotfr{\clC_1}$ is locally tabular, and so $\quotfr{\clC_1}$ is uniformly tunable. By Lemma \ref{lem:quotient-uniformly-tunable}, $\clC_1$
is uniformly tunable.  }

It follows that $\clC=\clC_0\cup\clC_1$ is uniformly tunable.
The formulas $B_h$ are known to be canonical \cite[Theorem 6.4]{Seg_Essay},
so $h(F_L)\leq 2$. By Theorem \ref{thm:supple-clusters-crit}, the logic of $F_L$ is locally tabular.  
Since $\Log F_L\subseteq L$, $L$ is locally tabular as well.
\end{proof}

==> store_pfmp_2024-12-28.tex <==
 A modal logic \(L\) has the \emph{product fmp}, if \(L\) is the logic of a class of finite product frames.
Like the local tabularity, the product fmp implies several desirable conditions.
For example, both local tabularity and the product fmp entail the fmp.
There are examples of logics having both properties, such as the product logics above~\(\LS5^2.\)
However, the connection between these two properties is unknown.
Some particular cases are described: for example, if~\(L_1\) is tabular and~\(L_2\) has fmp, then~\(L_1 \times L_2\) where has the product fmp \cite[Corollary~5.9]{MLTensor}.
By Corollary~\ref{cor:criterion-logics-general}, all such product logics are locally tabular.
In this section we describe two new sufficient conditions for the product fmp that hold for some locally tabular logics.

\begin{lemma}\label{lem:finite_preimage}
\hide{
 Let $L$ be a (uni)modal  \IS{not a product} logic with the followings properties:
 \begin{enumerate}
     \item $L$ is a pretranitive logic of finite height; 
     \item $L$ has a bounded cluster property. 
 \end{enumerate}
} 
Let $F$ be a pretransitive rooted frame of finite height with the bounded cluster property, $f:F\toto G$ with $G$ finite. 
Then there is a finite subset $U$ of $F$ such that 
$f\restr U: F\restr U\toto G$. 
\end{lemma}
\ISLater{$f\restr U$ - notation}
\begin{proof} 
Let \(F=(X,(R_\Di)_{\Di\in \AlA})\) and \(G=(Y,(S_\Di)_{\Di\in \AlA})\) be \(\Al\)-frames satisfying the assumptions. For any finite subset $V\subseteq X$, we define the {\em defects $D(V)$ of~$V$}:
\begin{gather*}
D_\Di(V)= \{a\in V\mid  \exists b\, (f(a) S_\Di b \, \text{ and for no } c \in V,\,
 a R_\Di c\, \& \, f(c)=b \},
 %D_\Di(V)= \{a\in V\mid  \exists b\, (f(a) S_\Di b \, \text{ and for no } c \in V,\,
 %(a R_\Di c \text{ and }  f(c)=b) \},
\\
D(V)=\bigcup\nolimits_{\Di\in\AlA} D_\Di(V) .
\end{gather*}
Observe that for any \(V\) with \(D(V) = \emp\) the restriction \(f\restr V\) satisfies the back condition.
%Since $f$ is a p-morphism, 
%for any finite \(V \subseteq X\) there exists a finite set $C(V)$ such that 
%for each $a\in X$ and  $b\in Y$ with  $f(a) S_\Di b$,  
%there is $c$ in $C(V)$ such that $a R_\Di c$ and $f(c)=b$.
%  One can readily see that if $V$ contains the root of~$\F$ and~$D(V)=\emp$, then 
% $f\restr V: F\restr V\toto G$; in particular,  $f\restr V$ is surjective, since $\G$ is rooted.
  Recall that \(\sim_F\) denotes the equivalence relation \(R_F^*\cap {R_F^*}\inv\). For any subset \(V \subseteq X\), let $C(V)=\bigcup\{[a]_{\sim_F} \mid a \in V\}$. 

  We define the sets $U_n\subseteq X$ for \(n \ge 0\) recursively. %and $V_n$ for $n<h$.  
 Let $U_0$  be the cluster of a  root of~$F$. For any \(n \ge 0,\) let \(V_n = C(R_F[D(U_n)])\) and
 \(U_{n+1} = U_n \cup V_n.\)
 It easily follows that~\(V_n\) is closed under~\(\sim_F\), and therefore so is \(U_n\) for all \(n\ge 0.\) Furthermore, \(V_n \subseteq R_F^*(u)\) for all \(u\in U_n.\) 

If~\(V_n\ne \varnothing,\) then \(D(U_n)\ne \varnothing,\) so for some modality~\(\Di\) there exists \(a\in U_n\) and~\(b\in R_\Di[f(a)]\) such that~\(f\inv(b)\cap U_n\cap R_\Di[U_n] = \varnothing.\) 
By the back condition of \(f\), there exists~\(c\in f\inv(b)\) such that \(a R_\Di c\).
Then~\(c\in V_n \setminus U_n\).
For any \(d\in U_n,\) we have \(c\in R_F^*(d)\). If~\(c R_F^* d\) for some~\(d\in U_n,\) then~\(c \sim_F d,\) so~\(c\in U_n\) since~\(U_n\) is closed under~\(\sim_F,\) a contradiction.
Then for any~\(n\) such that~\(V_n\ne \varnothing\) there exists a strict~\(R_F^*\)-chain in~\(F.\)
Since~\(F\) has finite height,~\(V_k = \varnothing\) for some~\(k < \omega.\)
 
 Let \(U = U_{k}.\)
 Assume that \(D(U_k) \ne \varnothing\), then \(R_F[f[U_k]] \ne \varnothing,\) so \(V_k \ne \varnothing\) by the back condition of~\(f\), a contradiction.
 It follows that~\(D(U_k) = \varnothing\), so the back condition holds for \(f\restr U\).
 Moreover, \(U_n\) are increasing with respect to inclusion, so \(U\) contains the root of \(F;\) since \(f\) is a p-morphism, \(f\restr U\) is surjective.
 It is trivial that \(f\restr U\) is a homomorphism.
 We conclude that \(f\restr U\) is a p-morphism.
 
% Claim: for $x\in D(U_{n-1})$, the depth of $f(x)$ is $G$ is less than $h-n$ (?ARITHMETIC),  
% Auxiliary claim:   $D(U_{n-1})\subseteq U_{n}$.
%for $x\in U_n{\setminus}U_{n-1}$, the depth of $x$ in $F$ is less than $h(F)-n$ (?ARITHMETIC). 
%It follows that $D(U_{h(G)})=\emp$, and we put $U=U_{h(G)}$. This completes the proof.
\end{proof}

\begin{proposition}
    Let \(F\) be a rooted pretransitive frame of finite height that has the bounded cluster property. If \(f:\:F \times G \toto H\) for some rooted frame \(G\) and a finite rooted frame \(H,\) then there exists a finite subframe \(F_1\) of \(F\) such that \(F_1 \times G \toto H.\)
\end{proposition}
\begin{proof}
    Let \(F = (X,(R_\Di)_{\Di\in \AlA})\) and \(G= (Y, (S_\Di)_{\Di\in \AlB})\). 
    Let \(H = (W, (\rho_\Di)_{\Di\in\AlA} \cup (\sigma_\Di)_{\Di\in \AlB});\) we will denote the relation \(\bigcup_{\Di\in \AlA} \rho_\Di\) by~\(\rho\) and \(\bigcup_{\Di\in \AlB} \sigma_\Di\) by~\(\sigma\).

    Let \(E = \rho^*(w_0),\) where \(w_0\) is the root of \(H,\) and let \(H_X\) be the reduct of \(H\restr E\) onto the horizontal relations: \(H_X = (E, (\rho_\Di)_{\Di\in\AlA}).\)
    We define a map \(f_X:\:X \to E\) by \(f_X(a) = f(a,b_0),\) where \(b_0\) is the root of \(F_Y.\) This map is well-defined since \(f\) is a homomorphism.
    We claim that \(f_X:\:F \toto H_X.\)
    It is trivial that \(f_X\) is a homomorphism.
    To show surjectivity, consider the root \(a_0\) of \(F.\)
    Since \(f\) is a p-morphism, \(f(a_0,b_0) = w_0\), then \(f_X(a_0) = w_0,\) so \(f_X\) maps \(a_0\) to the root of \(H_X\), therefore \(f_X\) is surjective. 
    Finally, for the back condition consider \(a\in X\) and \(w\in E\) such that \(f_X(a) \rho_\Di w\).
    We have \(f(a,b_0) = w,\) so there exists \(c\in X\times Y\) such that \((a,b_0) R_\Di^h (c,b_0)\) and \(f(c,b_0) = w.\) Then \(a R_\Di c\) and \(f_X(c) = w,\) as desired.

    By Lemma~\ref{lem:finite_preimage}, there exists a finite subset \(U \subseteq X\) such that \(f_X \restr U:\:F_1 \toto H_X\).

    We finish the proof by showing that \(f\restr (U\times Y)\) is a p-morphism from \(F_1 \times G\) to \(H.\)
    Again \(f\restr (U\times Y)\) is a surjective homomorphism, since it is a restriction of \(f\) and maps the root of \(F_1\times G\) to the root of~\(H.\) 
    Let us show the back condition.
    Let \(f(a,b) \rho_\Di v\) for some \((a,b)\in U\times Y\) and \(v\in W.\) 
    % Then \((a,b) R^v_\Di (c,b)\) for some \(c\in X\) such that \(f(c,b) = v.\)
    Then \((a,b_0) (R^v)^n (a,b) \) for some \(n < \omega.\)
    By the monotonicity of~\(f,\) \(f(a,b_0) \sigma^n f(a,b).\) Since \(H\) is a p-morphic image of a product frame, \(\rho_\Di\circ  \sigma^n = \sigma^n \circ\rho_\Di,\) so \(f(a,b_0) \rho_\Di u \sigma^n v.\)
    Then \(f_X(a) \rho_\Di u.\) Since \(f_X\restr U\) is a p-morphism, there exists \(c\in U\) such that \(a R_\Di c\) and \(f_X(c) = u\).
    Then \(f(c,b_0) = u\). Since \(u \sigma^n v,\) by the back condition of \(f\) there exists \(d\in Y\) such that \(b_0 R_G^n d\) and \(f(c,d) = u.\) Finally, notice that \((a,b) R^h_\Di (c,b)\)
    
    
    
    
    
    Since \(H\) is rooted, \(w_0 \rho^n u \sigma^k v\) for some \(u\in E\) and \(n,\,k< \omega.\)
    Then by the surjectivity of \(f_X\restr U\) there exists \(c\in U\) such that \(f_X(c) = u.\)
    Consequently, \(f(c,b_0) = u.\)
    By the back condition of~\(f\) there exists \((c,d)\in U\times Y\) such that \(b_0 R_G^k d\) and \(f(c,d) = u.\) Then \(\)
\end{proof}

A Kripke complete logic \(L\) is \emph{subframe}, if for any \(L\)-frame \(F,\) for any \(U \subseteq \dom F,\) the logic \(L\) is valid in the subframe \(F\restr U.\)
\ISLater{reconsider this}
 \begin{theorem}\label{thm:subframe}
   Let~\(L_X,\,L_Y\) be modal logics such that:
   \begin{enumerate}
       \item \(L_X\) is subframe;
       \item \(bc_m \in L_X\) for some~\(m \in \omega;\)
       \item \([B_h]^m \in L_X\) for some~\(h < \omega\);
       \item \(L_Y\) is pretransitive;
       \item \(L_X\times L_Y\) has finite model property.
     \end{enumerate}
  Then \(L_X\times L_Y\) has the product fmp.
\end{theorem}
\begin{proof}
    Let \(\clF_X\) and \(\clF_Y\) be the classes of finite rooted frames of \(L_X\) and \(L_Y\), respectively. 
\end{proof}


==> storeroom.tex <==
\newpage


\section{Old part for $\LS{5}^2$}

\input{subs-productivization}


\section{Old part for $\TL$}




\section{

\newpage 

\section{Questions and ideas:}
 
\begin{question}
Assume $L_0$ is canonical, $L$ its proper extension.
Is it possible that $\Log(F_{L})=L_0$?

If not, it would imply Lemma \ref{lem:ext-s5sq-canon} immediately.

But perhaps it is possible: seems that the logic of the canonical frame of $\GL$ is just $\LK{4}$.
\end{question}


\begin{question}
Is there a simple argument for  the Lemma \ref{lem:ext-s5sq-canon} or its substitute?
If $L$ is Kripke complete, $L_1$ is not, do we expect that there is a 
complete logic $L'$ with $L\subset  L'\subseteq L_1$? 

No! Take the logic $L$ of two-element chain, and an incomplete logic $L_1$ having only 
singletons as its rooted frames. 
\end{question}


\subsection{Locally tabular logics above $\LS{5}^n$}

\begin{theorem}
Assume that $L$ is an extension of $\LS{5}^n$. 
Then $L$ is not locally tabular if and only if 
$L\cap \ML(\Di_i)=L\cap \ML(\Di_j)=\LS{5}$ for some distinct $i,j$.  
\end{theorem} 
\begin{proof}
The `if' direction is trivial, since $\LS{5}^2$ is not locally tabular. 
\todo{The other direction is either trivial corollary of criterion or wrong. Do we need Kripke completeness?}
\end{proof}


\input{axiomatic-version}

\subsection{Products above $\LK{5}^2$}


~~~
\subsection{Products above $\Grz.3^2$}
~~~
\subsection{Products above the square of difference logic}

~~
\subsection{Products above the transitive logics of finite height}

What are locally tabular logics here?
What are not locally tabular Kripke complete logics here?

For example, let $L$ be the logic of two-level preorders (next step after $\LS{5}^2$).
What do we know about extensions of $L^2$? $L^2$ and $\LS{5}^2$ are not locally tabular. What else?
Perhaps, start with linearity first. There seems to be infinitely many non-locally tabular extensions of the square $L=(\LS{4.3}.B_2)^2$: different logics are produced by restricting the size of the top cluster/bottom cluster. There must be some doable systematization. What are maximal non-locally tabular (pretabular) logics above $L$?


\subsection{FMP}

$L_1$ has bounded cluster property, $L_2$ admits filtration. Does $L_1\times L_2$ admit filtration?

\section{Finite variable fragments}
When does k-finiteness of a product imply its local finiteness?
Seems yes for $k=1$.  

Seems that $k=2$ (or perhaps $k=1$) should be the case for products above $S4\times S4$.


\subsection{Chequered products}

What about the situation when valuations are restricted by finite unions of  rectangles?

Let $F=(X,R)$, $G=(Y,S)$.
A {\em rectangle} is a set of form
$A\times B$, $A\subseteq X$, $B\subseteq Y$.

This operation, $\bigotimes$ is, in some sense, more natural than product.

See \cite{MLTensor}.

\begin{question}
When the $\bigotimes$-product of uniformly tunable frames/locally tabular logics is uniformly tunable?
\end{question}

\ISH{It does not seem to be the case in general: $\LS{5}^2$ has the product finite model property; as far as I remember, it means that $\LS{5}\bigotimes \LS{5}=\LS{5}^2$. It looks like
this lead to a counterexample to the question. }






\subsection{Decolored products}

One modality corresponds to the union of the product modalities.





\subsection{Segerberg squares}
Add projections to the diagonal etc.

\newpage 
\section{Store room} 
$L_1$ is axiomatized above $\LS{4}$ by: height 2, linearity, $\Box\Di p\imp \Di \Box p$ (every cluster sees a maximal cluster, which is a singleton) 


Idea for $\hat{L}=L_1\times \LS{5}$: 
$\hat{L}$ is Kripke complete (known). 
Seems that it admits filtrations (it has heigth 2; filtrate clusters separately). 
Is every finite point-generated frame of $\hat{L}$ a p-morphic image of a finite button$\times$ $\mathbf{n}$ ? 


\begin{proof}[Temporary: sketch of the proof of pretabularity of $\LS{5}^2$ w.o. completeness argument.

Assume $L$ is an extension of $\LS{5}^2$. 

Firstly, we claim that if $L$ has no rpp axioms, then $L=\LS{5}^2$. 
If $L$ has no rpp axioms, then $F_L$ has no rpp, since rpp-axioms are canonical. 
Let $L_0=\Log(F_L)$. 
We have $\LS{5}^2\subseteq L_0\subseteq L$. 
Let $\clF$ be the class of point-generated subframes of $F_L$.
Then $L_0=\Log(\clF)$. So $\clF$ lacks rpp. By Proposition \ref{prop:rpp-factor}, 
$\fact{\clF}{\sim}$ lacks rpp as well. Then \ISH{known semantic argument for $\LS{5}^2$-frames which are products} the logic $L_1$ of the class  $\fact{\clF}{\sim}$ is $\LS{5}^2$. 
By Lemma \ref{lem:p-morph-sim}, $L_0\subseteq L_1$. 
So we have:
$$
\LS{5}^2 \subseteq L_0\subseteq L_1=\LS{5}^2
$$ 
\ISH{And what?...}
\end{proof}

\ISH{Strategy: 

Let \(\clF\) be a class of \(\LS{5}^2\)-frames such that \(\overline\clF\) is uniformly tunable. Then \(\clF\) is uniformly tunable.

Let \(\clF\) be a class of \(\LS{4}^2\)-frames such that \(\overline\clF\)  is uniformly tunable.  Is \(\clF\) is uniformly tunable?

\({\sim}\,=\,R_1\cap R_1\inv\cap R_2\cap R_2\inv\)

Let \(\clF\) be a class of commutative bimodal frames such that \(\overline\clF\)  is uniformly tunable. Is \(\clF\) is uniformly tunable?

(seems that the \(\sim\)-quotient is a sum)
}



\begin{proposition}\label{prop:supple-clusters-crit-only-if}
  If \(\Log(\clF)\) is locally tabular then \(h(\clF) \le h\) for some \(h < \omega\)  and $\clusters{\clF}$ is uniformly tunable.
\end{proposition}
\ISH{This follows from Theorems \ref{thm:1-finite-to-m-h} and \ref{prop:LF-for-subframess}, 
since the logic of all subframes is contained in the logic of clusters.}
\begin{proof}
  Let \(\Log(\clF)\) be locally tabular. Then \(\Log(\clF)\) is \(1\)-finite, so by Theorem~\ref{thm:1-finite-to-m-h} \(\Log(\clF)\) contains the formulas \(\Di_\AlA^{m+1} p \imp \Di_\AlA^{\leq m} p\) and
\( B_h^{[m]}\) for some~\(m,\,h < \omega.\) Then \(\clF\) is \(m\)-transitive and \(h(\clF) \le h.\)

  It remains to show that \(\clusters{\clF}\) is uniformly tunable. By Theorem~\ref{thm:LFviaTuned}, \(\clF\) is \(f\)-tunable for some \(f:\:\omega\to \omega.\) Let \(G\in \clusters{\clF}.\) Then \(G\) occurs as a cluster in some \(F \in \clF.\) Let \(\clU\) be a finite partition of \(G,\) then \(\clU\cup \{\dom F \setminus \dom G\}\) is a partition of \(F.\) Since \(F\in\clF,\) \(F\) is \(f\)-tunable, this partition has a tuned refinement~\(\clU'\)  with \(|\clU'| \le f(|\clU|+1).\) Then \(\clU'\restr G := \{U\in\clU'\mid U \subseteq \dom G\} \subseteq \clU'\) is a partition of \(\dom G\) that refines \(\clU,\) and \(\clU'\restr G\) is tuned in \(G.\) Since \(\clU'\restr G \subseteq \clU'\), \(|\clU'|\le f(|\clU|+1).\) Then \(\clusters\clF\) is \(g\)-tunable for \(g(n) = f(n+1).\)
\end{proof}

For the opposite direction  we will need the following lemmas.
\begin{lemma}\label{lem:disjoint-union-tunable}
  If \(f:\:\omega\to \omega\) is a monotonic function, and \(\{F_i\}_{i\in I}\) is a set of \(f\)-tunable \(\AlA\)-frames then the disjoint sum \(F = \biguplus_{i\in I} F_i\) is \(g\)-tunable, where
  \[
    g(n) = 2^{f(n)^2\cdot |\AlA|}\cdot n^{f(n)}\cdot f(n)^2.
  \]
\end{lemma}
\ISH{
There is a very simple argument for local finiteness of disjoint sums (I believe this is what we need): if the logic of a class of frames is locally tabular (or: class is $f$-tunable), 
then the logic of the class of their disjoint sums is (or tunability follows).

The estimation of $g$ tells us more. But I am not quite sure why does the size depend on $\Al$? Once we tuned the restriction of partitions on the components, it seems we are done... 
}
\begin{proof}
  Let \(F_i = (X_i,\,\{R_{i,\Di}\}_{\Di\in \AlA})\) for \(i \in I;\;F = (X,\,R).\) 

  For \(U \subseteq X,\) let \(\pi_i(U) = \{x\in X_i\mid (x,\,i)\in U\}.\)

  Let \(\clU = \{U_1,\,\ldots,\,U_n\}\) be a partition of \(X,\,|\clU|= n < \omega.\) Then \(\clU_i= \{\pi_i(U)\mid U\in \clU\}\) is a partition of \(X_i\) and \(|\clU_i|\le n\) for any \(i\in I.\) Find a tuned refinement \(\clU_i'\) of~\(\clU_i\) with \(|\clU_i'|\le f(n)\) for every \(i\in I.\)

  Let \(\AlA = \{\Di_1,\,\ldots,\,\Di_m\}.\) Define a signature 
  \[
    \Omega_n = \left(S_1^{(2)},\,\ldots,\,S_m^{(2)},\,P_1^{(1)},\,\ldots,\,P_n^{(1)},\,c\right)
  \]
  where \(S_1^{(2)},\,\ldots,\,S_m^{(2)}\) are binary relation symbols, \(P_1^{(1)},\,\ldots,\,P_n^{(1)}\) are unary relation symbols, and \(c\) is a constant.

  For every \((x,i)\in X,\) we define an \(\Omega\)-structure 
  \[
    \strA(x,i) = (S_1(i),\,\ldots,\,S_m(i),\,P_1(i),\,\ldots,\,P_n(i),\,q_{\clU'_i}(x)),
  \]
  where
  \begin{align*}
    S_k(i) &= \{(U,V)\mid U,\,V\in \clU'_i;\;\exists x\in U\,\exists y\in V\left(xR_k y\right)\} \subseteq 2^{\clU'_i \times \clU'_i},& k = 1,\,\ldots,\,m;\\
    P_l(i) &= \{U\in \clU'_i \mid U \subseteq \pi_i(U_l)\} \subseteq \clU_i,& l = 1,\,\ldots,\,n.
  \end{align*}
  Let \((x,i)\sim (y,j)\) iff the \(\Omega_n\)-structures \(\strA(x,i)\) and \(\strA(y,j)\) are isomorphic. We claim that \(\fact{X}{\sim}\) is a tuned refinement of \(\clU.\) 

  First observe that \((x,i)\in U_k\) iff \(q_{\clU'_i}(x)\in P_l(i)\) for any \((x,i)\in X\) and any \(l = 1,\,\ldots,\,n.\) 

  We show that \(\fact{X}{\sim}\) is a refinement of \(\clU.\) Suppose \((x,i)\sim (y,j)\) and \((x,i)\in U_l\) for some \(l.\) Then \(q_{\clU_i'}(x_i)\in P_l(i).\) Since \((x,i)\sim (y,j),\) there exists an isomorphism \(h:\:\strA(x,i)\to \strA(y,j).\) Since \(h\) preserves the relation \(P_l^{(1)},\)  \(h(q_{\clU_j'(x)})\in P_l(j);\) since \(h\) preserves the constant \(c,\) \(h(q_{\clU_i'}(x)) = q_{\clU_j'}(y).\) It follows that \( q_{\clU_j'}(y) \in P_l(j),\) so \((y,j)\in U_l.\)

  Fix any \(k = 1,\,\ldots,\,m\) and show that \(\fact{X}{\sim}\) is \(R_{\Di_k}\)-tuned. Let \((x,i) \sim  (y,j)\) and \((x,i) R (x',i').\) Then \(i=i'\) and \(x R_{i,\Di_k} x',\) so \(\left(q_{\clU'_i}(x), q_{\clU_i'}(x')\right)\in S_k(i).\) The structures \(\strA(x,i)\) and \(\strA(y,j)\) are isomorphic, so let \(h\) be the isomorphism. Then \(h(q_{\clU'_i}(x)) = q_{\clU'_j}(y)\) and \(\left(h(q_{\clU'_i}(x)), h(q_{\clU_i'}(x'))\right) = \left(q_{\clU'_i}(y), h(q_{\clU_i'}(x'))\right) \in S_k(j).\) Then some pair of points from \(q_{\clU'_j}(y)\) and \(h(q_{\clU'_i}(x'))\) is \(R_{j,\Di_k}\)-related. Since \(\clU'_j\) is \(R_{j,\Di_k}\)-tuned, \(y R_{j,\Di_k} y'\) for some \(y'\in h(q_{\clU'_i}(x')).\) Since \(q_j(y') = h(q_{\clU'_i}(x'))\), \(h\) is also an isomorphism between \(\strA(x',i) \) and \(\strA(y',j).\) Then \((x',i)\sim (y',j).\)

  Finally, \(\strA(x,i)\) has a finite carrier \(\clU_i'\) for every \((x,i)\in X.\) In an \(\Omega_n\)-structure on \(k\) elements, \(S_k(i)\) is interpreted as one of \(2^{k^2}\) binary relations on the carrier for \(k = 1,\,\ldots,\,m\) and, the constant \(c\) has \(k\) possible interpretations. An interpretation of \(P_1^{(1)},\,\ldots,\,P_n^{(1)}\) is a sequence of pairwise disjoint sets covering the carrier, so it corresponds to
  a function, so these interpretations are bijective to the functions  \(\{1,\,\ldots,\,k\} \to \{1,\,\ldots,\,n\}.\) Then the structures \(\strA(x,i)\) with \(|\clU'_i| = k.\) form at most \(\left(2^{k^2}\right)^m \cdot n^k \cdot k\) isomoprhism classes. Since \(|\clU_i'|\le f(n)\) for every \(i\in I,\)
  \[
    \left|\fact{X}{\sim}\right| \le \sum_{\exists i\in I:\:k=|\clU'_i|}\left(\left(2^{k^2}\right)^m \cdot n^k \cdot k\right) \le \sum_{k=1}^{f(n)} 2^{k^2m} \cdot n^k \cdot k = \left(2^{k^2|\AlA|}\right) \cdot n^k \cdot k.
  \]
\end{proof}




\begin{proof}[Original proof of Lemma \ref{lem:generated-subframe-tunable}]
  Let \(\clU\) be a partition of \(\dom F,\,|\clU| = n < \omega.\) Then \(\clU\) induces partitions \(\clU_1,\,\clU_2\) of \(X_1\) and \(X_2,\) respectively. Let \(\clU'_1\) be a tuned refinement of \(\clU_1\) such that \(|\clU'| \le f(|\clU'_1|) \le f(n).\) 

  Let \(\AlA = \{\Di_1,\,\ldots,\,\Di_m\}.\) Define \(\alpha_k:\:X_2  \to 2^{\clU'_1}\) by 
  \[
    \alpha_k(x_2) = \{U\in \clU'_1 \mid x\in R_{\Di_k}\inv(U)\},\quad x\in X_2,\,k = 1,\,\ldots,m.
  \]
  The map \(x \mapsto (q_{\clU_2}(x),\,\alpha_1(x),\,\ldots,\,\alpha_m(x))\) induces a refinement \(\clU_2'\) of \(\clU_2,\) and
  \[
     |\clU_2'| \le |\clU_2| \cdot \left(2^{|\clU_1'|}\right)^n \le f_1(n) \cdot 2^{f_1(n)\cdot m} < \omega.
   \]
   Then there exists a tuned refinement \(\clU_2''\) of \(\clU_2'\) of size at most \(f_2\left(2^{f_1(n)\cdot m}\right).\) 

   The partition \(\clB = \clU_1' \cup \clU_2''\) is a refinement of \(\clU.\) We claim that it is tuned.

   Let \(xR_{\Di_k} y\) for some \(x,\,y\in X\) and \(\Di_k\in \AlA,\) and let \(x'\in q_\clB(x).\) Find \(y'\in q_{\clB}(y)\) such that \(x' R_\Di y'.\)

   If \(x\in X_1\) then \(y\in X_1\) since \(F\restr X_1\) is a generated subframe. Then \(x\) and \(x'\) belong to the same block of \(\clU_1'.\) Since \(U_1'\) is tuned, \(x' R_{\Di_k} y'\) for some \(y\in q_{\clU_1'}(y).\) But then \(y'\in q_{\clB}(y),\) as desired.

   Now assume \(x\in X_2,\) then \(x'\in q_{\clU_2''}(x)\) and \(\alpha_k(x) = \alpha_k(x').\)If \(y\in X_1\) then \(q_{\clU_1'}(y)\in \alpha_k(x) = \alpha_k(x'),\) so  \(x'\in R_{\Di_k}\inv(q_{\clU_1'}(y)),\) as desired. If \(y\in X_2\) then \(x' R_{\Di_k} y'\) for some \(y'\in q_{\clU_2''}(y)\) since \(\clU_2''\) is tuned. 

   Finally,
   \[
     |\clB| \le |\clU_1'| + |\clU_2''| \le f_1(n) + f_2\left(2^{f_1(n)\cdot m}\right).
   \]
\end{proof}


\begin{lemma}\label{lem:height-clusters-tunable}
  Fix an alphabet \(\AlA.\) Given \(f:\:\omega\to \omega\) and \(1\le h < \omega,\) let \(\clF_{h,f}\) be the class of \(\AlA\)-frames 
  \[
    \clF_{h,f} = \left\{F\mid h(F) \le h,\,\clusters{\{F\}} \text{ is }f\text{-tunable}\right\}.
  \]
  Then \(\clF_{h,f}\) is uniformly tunable. 
\end{lemma}
\begin{proof}
  Fix a function \(f.\) Without loss of generality, we may assume that \(f\) if monotone. Show by induction on \(h\) that \(\clF\) is uniformly tunable.

  For the base case, let \(h = 1,\) then any frame \(F\in \clF_{1,f}\) has height \(1,\) so \(F\) is a disjoint union of clusters. By Lemma~\ref{lem:disjoint-union-tunable}, \(F\) is \(g_1\)-tunable for \(g_1(n)=2^{f(n)^2\cdot |\AlA|}\cdot n^{f(n)}\cdot f(n)^2.\) Then \(\clF_{1,f}\) is \(g_1\)-tunable.

  To show the transition, assume that \(\clF_{h,f}\) is \(g_h\)-tunable for some monotone \(g_h:\:\omega\to\omega\). Let \(F\in \clF_{h+1,f}.\) Let \(h(F) = h+1.\) Let \(X_1\) be the union of all maximal clusters in \(F;\) let \(X_2 = \dom F \setminus X_1.\) Then \(F\restr X_1\) is a disjoint union of clusters, and a generated subframe of \(F.\) By Lemma~\ref{lem:disjoint-union-tunable}, \(F\restr X_1\) is \(g_1\)-tunable. By hypothesis, \(F\restr X_2\) is \(g_h\)-tunable. Then Lemma~\ref{lem:generated-subframe-tunable} implies that \(F\) is \(g\)-tunable where
  \[
    g(n) = g_1(n) + g_h\left(n\cdot 2^{g_1(n)\cdot |\AlA|} \right) \ge g_h(n).
  \]
   If \(h(F) \le h\) then \(F\) is \(g_h\)-tunable by hypothesis. Since \(g_h\le g,\) \(F\) is \(g\)-tunable. Therefore \(\clF_{h+1,f}\) is uniformly tunable, as desired.
\end{proof}

\begin{proposition}\label{prop:supple-clusters-crit-if}
  If $\clF$ is a class of \(\AlA\)-frames of uniformly finite height and $\clusters{\clF}$ is uniformly tunable, then \(\clF\) is uniformly tunable.
\end{proposition}
\begin{proof}
  Let \(h(\clF) = h\) and find \(f:\:\omega\to \omega\) such that \(\clusters{\clF}\) is \(f\)-tunable. Then \(\clF\subseteq \clF_{h,f}.\) By Lemma~\ref{lem:height-clusters-tunable}, \(\clF\) is uniformly tunable.
\end{proof}



\begin{theorem}\label{SRthm:criterion-frames-rpp} 
Let $\clF$ and $\clG$ be non-empty classes of $\AlA$- and $\AlB$-frames, respectively. 
TFAE:
\begin{enumerate}[(i)]
\item The logic $\Log(\clF\times \clG)$  is locally tabular;
\item The logics $\Log(\clF)$ and $\Log(\clG)$ are locally tabular, 
and $\clF\times \clG$ has the rpp.
\end{enumerate}
\end{theorem}

\begin{theorem}\label{SRthm:criterion-rpp1} Let $L_1, L_2$  be Kripke complete consistent logics.
TFAE:
\begin{enumerate}[(i)]
\item $L_1\times L_2$  is locally tabular;
\item 
$L_1$ and $L_2$ are locally tabular and  $L_1\times L_2$ contains a formula 
$\RP_m(\AlA)$ for some $m$; here $\AlA$ is the alphabet of modalities of $L_1\times L_2$.
\end{enumerate}
\end{theorem}

\begin{proposition} For an $\Al$-frame $F$, 
$(\dom{F},R_F)$ satisfies $\RP_m$ iff 
$F\mo \RP_m(\Di_\AlA)$.
\end{proposition}
\begin{proof}
Straightforward.\ISH{later: double check again}
\end{proof}

\begin{theorem}\label{SRthm:criterion-frames} 
Let $\clF$ and $\clG$ be non-empty classes of $\AlA$- and $\AlB$-frames, respectively. 
TFAE:
\begin{enumerate}[(i)]
\item The logic $\Log(\clF\times \clG)$  is locally tabular;
\item The logics $\Log(\clF)$ and $\Log(\clG)$ are locally tabular, 
and at least one of the classes $\clF$, $\clG$ has 
the bounded cluster property.
\end{enumerate}
\end{theorem}
\begin{proof}
\ISH{Use proof of \ref{thm:criterion0}. Theorem should be corollary. }
\end{proof}
 




\begin{proposition}\label{SRprop:product-preserve-pretrans}~
\begin{enumerate}
  \item If $F$ is $m$-transitive and $G$ is $n$-transitive, then $F\times G$ is $(m+n)$-transitive.
  \item If $\clF$ and $\clG$ are pretransitive, then $\clF\times \clG$ is pretransitive.
  % \ISH{Was not defined. Perhaps, we do not need it at all, just the next proposition}
  \item The product of two pretransitive logics is pretransitive.
\end{enumerate}
\end{proposition}
\begin{proof}
  \begin{enumerate}
    \item Let \(F = \left(X,\,(R_\Di)_{\Di\in\AlA}\right),\,G = \left(Y,\, (S_\Di)_{\Di\in \AlB}\right).\) By hypothesis we have 
    \begin{equation}\label{eq:product-preserve-pretrans}
      \forall k < \omega,\quad {R_F}^k \subseteq {R_F}^{\le m},\ {S_G}^k  \subseteq {S_G}^{\le n}.
    \end{equation}
    Let \((a,b),\,(c,d)\in X\times Y\) and \((a,b)R_{F\times G}^*(c,d).\) Then \(a (R^h)^k c\) and \(b (R^v)^l d\) for some \(k ,\,l < \omega.\) 
    % \ISH{We use $a,b$ for elements of frames, it is better to use $i,j,k$ for natural}
    Then \(a  {R_F}^k c\) and \(b {S_G}^l d.\) By \eqref{eq:product-preserve-pretrans}, \(a {R_F}^{\le m} c\) and  \(b {S_G}^{\le n} d.\) Then
    \[
      (a,b) (R^h)^{\le m} (c,b) (R^v)^{\le n} (c,d).
    \]
    Since \(R^h,\,R^v \subseteq R_{F\times G},\) we have \((a,b) (R_{F\times G})^{\le m+n} (c,d).\) 

    Therefore \(R_{F\times G}^* \subseteq {R_{F\times G}}^{\le m+n}.\)
    \item Let \(F\times G \in \clF \times \clG.\) Then \(F\) and \(G\) are pretransitive; find \(m,\,n < \omega\) such that \(F\) is \(m\)-transitive and \(G\) is \(n\)-transitive. By (i) \(F\times G\) is \((m+n)\)-transitive, hence pretransitive. Since \(F\times G \in \clF \times \clG\) was arbitrary, \(\clF \times \clG\) is pretransitive.
    \item Let \(L_1,\,L_2\) be pretransitive. Find \(m,\,n\) such that \(L_1\) is \(m\)-transitive and \(L_2\) is \(n\)-transitive. Then \(\Frames(L_1)\) is \(m\)-transitive and \(\Frames(L_2)\) is \(n\)-transitive, so \(\Frames(L_1)\times\Frames(L_2)\) is pretransitive by (ii). Find \(k\) \ISH{$k=m+n$?}such that \(\Frames(L_1)\times\Frames(L_2)\) is \(k\)-transitive. Then
    \[
      L_1\times L_2 \vd \Di_\AlA^{k+1} p \imp \Di_\AlA^{\leq k} p,
    \]
    so \(L_1\times L_2\) is \(k\)-transitive, hence pretransitive by the definition.

  \end{enumerate}
\end{proof}



\begin{corollary}\label{cor:quotient-logic-inclusion}
Assume that in every $F$ in a  class $\clF$ of $\Al$-frames all relations are transitive. 
  Then~\(\Log{\clF} \subseteq \Log{\quotfr{\clF}}.\)
\end{corollary}
\ISH{Do we use this corollary?}



\ISH{In the following statement, we say ``of a Kripke complete proper extension of $\LS{5}^2$''. This might be misleading, since all of them are. I tuned it a bit.}
\begin{lemma}\label{SRlem:ext-s5sq-complete-old}
The class of frames of a Kripke complete proper extension of $\LS{5}^2$
is uniformly tunable.
\end{lemma}

 
\begin{proof}
  Let \(\clF\) be a class of point-generated \(\LS{5}^2\)-frames such that \(\Log{\clF} \supsetneq \LS{5}^2.\) Find  \(n = \sup\left\{m< \omega \mid \exists F\in\clF\ \left(\quotfr{F}\toto \rect{m}{m}\right)\right\}.\)

  Then \(n < \omega\) since otherwise \(\Log{\quotfr{\clF}} \subseteq\Log\{\rect{m}{m}\mid m < \omega\} = \LS{5}^2,\) and by Corollary~\ref{cor:quotient-logic-inclusion} \(L \subseteq \Log{\quotfr{\clF}} \subseteq \LS{5}^2.\)  By Lemma~\ref{lem:s5-square-quotient}, \(\quotfr{\clF} \subseteq \clF_1 \cup \clF_2,\)
   where \(\clF_i\) is the class of rectangle frames \(\{\rect{\kappa_1}{\kappa_2}\mid \kappa_i \le n\},\,i = 1,\,2.\) 
   \ISH{Now it is simpler: follows from Theorem \ref{thm:criterion-frames}. } 

   Observe that~\(\clF_1 \models \LS{5} \times (\LS{5}+Alt_n)\) where
   \[
     Alt_n = \Box\bigvee_{i \le n} p_i \to \bigvee_{i \le n}\bigvee_{j < i} \Di (p_i\land p_j)
   \]
   is the formula that defines the frame condition \(\forall x\:(|R(x)|\le n).\)

   By Theorem~\ref{thm:criterion0}, \(\Log \clF_1\) is locally tabular since \(\LS{5}+Alt_n\) has the bounded cluster property. Analogously, \(\Log\clF_2 \supseteq (\LS{5}+Alt_n) \times \LS{5}\) is locally tabular.

   Since \(\quotfr{\clF} \subseteq \clF_1 \cup \clF_2\), \(\Log \quotfr{\clF} \supseteq \Log \clF_1\cap \Log \clF_2\) is locally tabular. Then \(\Log{F}\) is locally tabular by Lemma~\ref{lem:quotient-uniformly-tunable}.
\ISH{We will later collect basic facts about local finiteness in preliminaries: extensions, intersections of finitely many, etc.} 

\end{proof}



If \(\kappa,\,\kappa',\,\mu,\,\mu'\) are cardinals, is easy to check that \(\rect{\kappa}{\mu}\toto \rect{\kappa'}{\mu'}\) whenever \(\kappa' \le \kappa\) and \(\mu' \le \mu.\) 

\begin{theorem}\cite{SR:Segerberg2DimML}
  \(\LS5^2 =\Log(\{\rect{m}{m} \mid m < \omega\}).\)
\end{theorem}






\section{Old (March 26) Preliminaries}\label{sec:prel}


\todo{To define: Logic; product; commutator; Local tabularity; }


For the basic notions in modal logic, see, e.g., \cite{CZ,BDV}.

\subsection{Modal syntax} Let $\Al$ be a finite set, an {\em alphabet of modalities}.
%We will always assume that $\Al$ is finite.
{\em Modal formulas over $\AlA$}, $\ML(\AlA)$ in symbols, are constructed from
a countable set of {\em variables} $\PV=\{p_0,p_1,\ldots\}$ using Boolean connectives $\bot,\imp$ and unary connectives $\Di\in \AlA$.
Other logical connectives are defined as abbreviations in the standard way, in particular $\Box\vf$
denotes $\neg \Di \neg \vf$. 

The term {\em unimodal} refers to the case when $\AlA$ is a singleton.

Define the following abbreviations: $\Di^0 \vf=\vf$,
$\Di^{i+1}\vf=\Di^i\Di\vf$,
$\Di^{\leq m} \vf =
\bigvee_{i\leq m} \Di^i \vf$, $\Box^{\leq m} \vf =\neg \Di^{\leq m} \neg \vf$.
We write $\DiAl\vf$ for $\bigvee_{\Di\in\Al}\Di \vf$.

A subset \(L \subseteq \ML(\AlA)\) is a {\em normal modal logic} if
\begin{enumerate}
  \item \(L\) contains all propositional tautologies,
  \item \((\Box p \land \Box(p \to q) \to \Box q)\in L\) for any \(\Box\) in the language \(\ML(\AlA),\)
  \item \(\Di p \lra \lnot \Box \lnot p \in L\) for any \(\Di\) in the language \(\ML(\AlA),\)
  % \ISH{By the way, Vlad, this definition is wrong! It does not work when $\Box$ is an abbreviation }
\end{enumerate}
and \(L\) is closed under the rules \(\mathbf{MP},\,\mathbf{Gen},\,\mathbf{Sub}\):
\begin{description}
  \item[(MP)] If \(\varphi,\,\varphi \to \psi \in L\) then \(\psi \in L,\)
  \item[(Gen)] If \(\phi \in L\) then \(\Box \varphi \in L\)  for any \(\Box\) in the language \(\ML(\AlA),\)
  \item[(Sub)] If \(\varphi \in L\) then for any \(p\in \PV\) and any formula \(\psi\in \ML(\AlA),\) the substitution of \(\psi\) for \(p,\) denoted \(\varphi\left(\frac{\psi}{p}\right)\), is contained in \(L.\)
\end{description}

Given an alphabet \(\AlA,\) an {\em \(\AlA\)-frame} is a pair \(F = (X,\,(R_\Di)_{\Di\in \AlA})\) where \(X\) is a \ISH{non-empty?} set and \(R_\Di \subseteq X\times X\) for any \(\Di\in \AlA\). In this case we denote \(\dom F = X\) and~\(R_F = \bigcup_{\Di\in \AlA} R_\Di.\)
By the cardinality $|F|$ of $F$ we mean the cardinality of its domain.
For $a\in X$, $Y\subseteq X$, we put $R_\Di(a)=\{b\mid aR_\Di b\}$,
$R_\Di[Y]=\bigcup_{a\in Y} R_\Di(a)$.


An \(\AlA\)-model is a pair \((F,\,\theta)\) where \(F\) is an \(\AlA\)-frame and \(\theta:\:PV \to \clP(X)\)
maps the propositional variables to subsets of \(X;\) such function is called a {\em valuation in \(F\)}.  We write \((F,\,\theta),a\models \varphi\) if \(\varphi\) is true at \(a\in \dom F\) under the valuation \(\theta.\) Accordingly, \((F,\,\theta) \models \varphi\) means that \(\varphi\) is {\em true in the model} \((F,\,\theta)\), and \(F\models \varphi\) means that \(\varphi\) is {\em valid in the frame}~\(F\). The notions of truth and validity are standard; see, for example, \cite{CZ}. In particular, 

\[
  (F,\,\theta),\,a\models \Di \varphi \iff (F,\,\theta),\,b\models \varphi\text{ for some }b\in R_\Di(a),\quad \Di\in \AlA.
\]

We put $$\vext(\vf)=\{a\mid (F,\v),a\mo\vf\}.$$

If \(\Gamma \subseteq \ML(\AlA)\) is a set of formulas, \((F,\,\theta)\models \Gamma\) \ISH{it is 'true'; but do we use it?} and \(F\models \Gamma\) denotes the validity of \(\Gamma\) in the model \((F,\,\theta)\) and in the frame \(F,\) respectively.

We define the {\em logic} \(\Log{(F,\,\theta)}\) of an \(\AlA\)-model \((F,\,\theta)\) as the set of all \(\AlA\)-formulas that are true in \((F,\,\theta)\).\ISH{It is not a logic, in general.}  The logic \(\Log{F}\) of a frame \(F\) is the set of all \(\AlA\)-formulas that are valid in \(F\). The logic \(\Log{\clF}\) of a class of frames \(\clF\) is the set of forumlas that are valid in all frames of \(\clF\). For a set of formulas \(\Gamma \subseteq \ML(\AlA),\) \(\Frames(\Gamma)\) is the class of \(\AlA\)-frames where \(\Gamma\) is valid.



\subsection{Quotient frame}
For a frame \(F = (X,\,(R_\Di)_{\Di\in A})\) and an equivalence $\approx$ on $F$, 
the {\em quotient frame} $\fact{F}{\approx}$ is the structure 
$(\fact{X}{\approx},\,(R^\approx_\Di)_{\Di\in\Al})$ where 
  \[
    [a] R^\approx_\Di [b] \iff \exists a'\in[a]\ \exists b'\in [b]\ \left(a' R_{\Di} b' \right),\quad \Di\in \AlA.
  \]

\subsection{p-morphisms}
  Let \(F = (X,\,(R_\Di)_{\Di\in \AlA}\) and \(G = (Y,\,(S_\Di)_{\Di\in \AlA})\) be \(\AlA\)-frames. A map \(f:\:X\to Y\) is a {\em p-morphism from \(F\) to \(G\)}, if it is
  \begin{enumerate}
    %\item surjective;
    \item monotone: for any \(a,\,b\in X\) and \(\Di\in \AlA,\) \(a R_\Di b\) implies \(f(a) S_\Di f(b)\) 
    \item lifting\ISH{Is it a good term?}:  for any \(a\in X,\,u\in Y\) and \(\Di\in \AlA,\) \(f(a) S_\Di u\) implies that there exists \(b\in X\) such that \(a R_\Di b\) and \(f(b) = u.\) 
  \end{enumerate}
  If $f$ is surjective,  we write \(f:\:F\toto G.\) If there exists a p-morphism from \(F\) onto~\(G,\) we write \(F \toto G.\) 

  It is well-known that \(F \toto G\) implies \(\Log{F} \subseteq \Log{G}.\)
\subsection{Products}


Let $\AlA$ and $\AlB$ be two disjoint finite sets. 
%\ISH{Later: say about the case $\AlA=\AlB$ that we shift modalities} 
%\newcommand\prod[1]{{#}
% \ISH{alternative version of product}
For an \(\AlA\)-frame \(F=\left(X,\,(R_\Di)_{\Di\in \AlA}\right)\) and \(\AlB\)-frame \(G = \left(Y,\,(R_\Di)_{\Di\in \AlB}\right)\), the {\em product frame} \( F\times G\) is the frame $(X\times Y,\,(R^h_\Di)_{\Di\in \AlA}, (R^v_\Di)_{\Di\in \AlB})$,  where 
\begin{align*}
    R^h_\Di&=\{((a,\,b),\,(a',\,b))\mid a,\,a'\in X,\,b\in Y,\,a R_\Di a'\}  &\text{ for }\Di\in \AlA;\\
    R^v_\Di &= \{((a,\,b),\,(a,\,b'))\mid a\in X,\,b,\,b'\in Y,\,b R_\Di b'\}  &\text{ for }\Di\in \AlB.
\end{align*} 
We say that relations $R^h_\Di$ induced by relations in $F$ are {\em horizontal},  and $R^v_\Di$ are {\em  vertical}; \ISH{What is more convenient in proofs: horizontal/vertical or induced?}
so $F\times G$  has $|\AlA|$ horizontal and $|\AlB|$ vertical relations.

\hide{
The product frame \(F\times G\) is an \((\AlA\sqcup\AlB)\)-frame.
\ISH{Earlier, $a,b$ were used for elements of frames. Now we have different notation. 
I think it is OK (if only we do not use first-order formulas extensively), but should be consitent through the text.} 
}

We use the notation \(R^h\) for \(\bigcup_{\Di\in \AlA} R_\Di^h\) and \(R^v\) for \(\bigcup_{\Di\in \AlB} R_\Di^v\)
\ISH{When possible, let us minimize the conventions. Do we need $R^h, R^v?$}

%\ISH{Or: $R^\times_\Di$ for product relations?}

For a class \(\clF\) of \(\AlA\)-frames and a class \(\clG\) of \(\AlB\)-frames, we put
\[
  \clF \times \clG = \{F\times G \mid F\in \clF,\,G\in\clG\}.
\]

If \(L_1 \subseteq \ML(\AlA)\) and \(L_2 \subseteq \ML(\AlB)\) are modal logics, the {\em product logic \(L_1\times L_2\)} is defined as
\[
  L_1\times L_2 = \Log(\{F\times G \mid F\models L_1,\,G\models L_2\}).
\]
If $L_1$ and $L_2$ are unimodal logics, we shift their modalities and follow the convention that
the alphabet $L_1\times L_2$ is $\{\Di_1,\Di_2\}$. \ISH{Sounds clumsy?}

\subsection{Local tabularity}
Let \(L\subseteq \AlA\) \ISH{typo} be a modal logic.
Define an equivalence relation \(\sim_L\) on \(\ML(\AlA)\) by 
\[\varphi \sim_L \psi \iff L \vd \varphi \lra \psi.\]

Given a number \(k < \omega,\) denote \(L\restr k\) the subset of \(L\) composed of all formulas that contain only the first \(k\) propositional variables from \(p_0,\,\ldots,\,p_{k-1}.\) 

For any \(k < \omega,\) a logic \(L\) is {\em \(k\)-finite} if \(L\restr k\) contains finitely many equivalence classes of formulas with respect to \(\sim_L.\)

A logic \(L\) is {\em locally tabular} if \(L\) is \(k\)-finite for any \(k < \omega.\)





   
\begin{proposition}\label{prop:product-preserve-height}
Assume that for some finite $h_1, h_2$, $h(\clF)=h_1$ and $h(\clG)=h_2$.
Then $h(\clF\times \clG)=h_1+h_2-1$.
\end{proposition}
\begin{proof}
  Find \(F\in \clF\) with \(h(F) = h_1\) and \(G\in \clG\) with \(h(G) = h_2.\) Find a chain \([a_0] < [a_1] < \ldots < [a_{h_1}]\) in \(\Sk F\) and a chain \([b_0]< [b_1] < \ldots < [b_{h_2}]\) in \(\Sk G.\) Then
  \[
    [(a_0,\,b_0)] < [(a_1,\,b_0)] < \ldots < [(a_{h_1},\,b_0)] < [(a_{h_1},\,b_1)] < \ldots < [(a_{h_1},\,b_{h_2})]
  \]
   is a chain of \(h_1 + h_2 - 1\) elements in \(\Sk (F\times G).\)

   By the definition, \(h(F\times G) = h_1 + h_2 -1,\) so \(h(\clF\times \clG) \ge h_1 + h_2 - 1.\)

   Assume for contradiction that $h(\clF\times \clG)\ge h_1+h_2,$ then there exists  a chain \(C\) of height \(h_1 + h_2\) in \(\clF\times \clG:\)
   \[
     [(a_0,\,b_0)] < [(a_1,\,b_1)] < \ldots < [(a_{h_1+h_2},\,b_{h_1+h_2})]
   \]
    in \(\Sk(F\times G).\) Then \(a_i R_F a_{i+1}\) or \(b_i R_G b_{i+1}\) for any \(i < h_1 + h_2.\) By the pigeonhole principle, \(C\) has a subchain of height \(h_1+1\) where all elements are related by \(R^h\) or a subchain of height \(h_2 + 1\) where all elements are related by \(R^v.\) In the former case, the first coordinates of the elements of this subchain form a chain in \(\Sk F,\) so \(h(F) \ge h_1 + 1,\) hence \(h(\clF)\ge h_1 + 1.\) In the latter case \(h(\clG) \ge h_2 + 1\) analogously.
\end{proof}




\paragraph{Local tabularity.}


Let \(L\subseteq \AlA\) \ISH{typo} be a modal logic.
Define an equivalence relation \(\sim_L\) on \(\ML(\AlA)\) by 
\[\varphi \sim_L \psi \iff L \vd \varphi \lra \psi.\]

Given a number \(k < \omega,\) denote \(L\restr k\) the subset of \(L\) composed of all formulas that contain only the first \(k\) propositional variables from \(p_0,\,\ldots,\,p_{k-1}.\) 

For any \(k < \omega,\) a logic \(L\) is {\em \(k\)-finite} if \(L\restr k\) contains finitely many equivalence classes of formulas with respect to \(\sim_L.\)

A logic \(L\) is {\em locally tabular} if \(L\) is \(k\)-finite for any \(k < \omega.\)








   \subsection{Olds statements about tuned}

   
\begin{theorem}\cite{LocalTab16AiML}\label{thm:LFviaTuned}
The logic of a class  $\clF$ of $\Al$-frames is locally tabular
iff $\clF$  is uniformly tunable.
\end{theorem}



For a frame \(F = (X,\,(R_\Di)_{\Di\in \AlA})\)  and \(Y \subseteq X\), put \(F\restr Y = (Y,\,(R_\Di\restr Y)_{\Di\in\AlA})\), where $R_\Di\restr Y= R_\Di\cap (Y\times Y)$.
For a class $\clF$ of  frames, put
  $$\SubFrs{\clF}=\{\frF\restr Y\mid \frF\in \clF \text{ and } \emp\neq Y\subseteq \dom{\frF}\}.$$
  %\ISH{Convention: do we exclude the empty frame? Let us do it.}

\begin{proposition}\cite{LTViaSums2022}\label{prop:LF-for-subframess}
If the logic of a class $\clF$ of $\Al$-frames is locally tabular,
then the logic of $\SubFrs{\clF}$ is locally tabular.
\end{proposition}\ISH{State for $k$-finite}


A frame $F$ is a {\em cluster}, if $a R_F^* b$ for all $a,b$ in $F$. 
For a class $\clF$ of frames, $\clusters{\clF}$ is the class of cluster-frames which are restrictions on clusters (as sets) occurring in frames in $\clF$:
%$\clusters{\clF}$ denotes the class of cluster-frames occurring as subframes in frames in $\clF$:
$$
\clusters{\clF}=\{F\restr C\mid C \text{ is a cluster in } F\in\clF\}
$$
\ISH{Do we need it? - 
For a logic $L$, let $\clusters{L}$ be the class of clusters occurring in its frames.
}
\begin{theorem}\cite{LocalTab16AiML}\label{thm:SR:supple-clusters-crit}
A logic $\Log(\clF)$ is locally tabular iff
$\clF$ is of uniformly finite height and $\Log\clusters{\clF}$ is locally tabular.
\end{theorem}
The proof of this theorem has not been given for the polymodal case, although it is a straightforward generalization of the proof of Theorem 5.2 in \cite{LocalTab16AiML}. For the sake of rigor, we consider the polymodal case in Appendix. 



 \subsection{Old abstract} 
 

We give the following criterion of local finiteness for products of Kripke complete modal logics. 

For a logic $L$, let $\clusters{L}$ denote the class of clusters occurring in its
frames (clusters are defined w.r.t. the transitive reflexive closure of the union of relations in a frame).  $L$ is said to have the {\em bounded cluster property}, if for some finite $m$, $|C| < m$ for all $C$ in $\clusters{L}$.  
Let $L_1, L_2$  be Kripke complete consistent logics.
We show that the product $L_1\times L_2$ is locally tabular iff 
$L_1$ and $L_2$ are locally tabular and at least one of these logics has
the bounded cluster property. 

==> tack2_alternative_and_remark.tex <==

\IS{Seems that we do not need it anymore. But we need to keep the footnote somehow... }


\begin{lemma}\label{lem:ext-TL-complete-store}
Let $\clF$ be a class of bimodal frames such that $\Log\clF$ is a proper 
extension of $\TL_2$. Then $\Log\clF$
is locally tabular.
\end{lemma}
\begin{proof}
Let \(\clG\) be the class of point-generated subframes of frames in $\clF$.
By Lemma \ref{lem:rootelTLframes}, every frame in $\clG$ is isomorphic to  $C\oplus \circ$ for an $\LS{5}^2$-cluster $C$. 
Let $\clC$ be the class of all such frames. 
Since $\Log\clF=\Log\clG$ is a proper 
extension of $\TL_2$,  then, in view of Lemma \ref{lem:LT-invariance}, $\Log(\clC)$  is a proper extension of 
$\LS{5}^2$. By Theorem \ref{thm:S5Nick}, 
the logic $L$ of this class is locally finite. So $\clC$ is a uniformly tunable class. Clearly, the top clusters in $\TL$-frames also form a uniformly tunable class, since they are singletons. Now the statement follows from Theorem 
\ref{thm:supple-clusters-crit}.
\end{proof}
\begin{remark}
For a Kripke complete proper extension $L$ of $\LS{5}^2$, local tabularity can be obtained directly,  as a  corollary of  
Theorem \ref{thm:criterion-frames-general}.
%and observations in  Section \ref{subs:Prod}. 
Indeed, let $\clF$ 
be the class of point-generated frames of $L$.
By Lemma~\ref{lem:p-morph-sim}, $L \subseteq \Log{\quotfr{\clF}}$.  
So $\Log{\quotfr{\clF}}$ is a proper extension of $\LS{5}^2$ as well, and hence \(n = \sup\{m  \mid \exists F\in\clF\  \,(\quotfr{F}\toto \rect{m}{m} )\}\) is finite. 
For \(i = 1,\,2\), let $\clG_i$  
be the class of frames of form $\rect{X_1}{X_2}$ with $|X_i|\leq n$. 
By Lemma~\ref{lem:s5-square-quotient}, 
each frame in  $\quotfr{\clF}$ is isomorphic to a frame in $\clG_1 \cup \clG_2$. 
   Both classes $\clG_i$ are uniformly tunable by Theorem~\ref{thm:criterion-frames-general},
   and so is the class $\quotfr{\clF}$.\footnote{This is a particular case of the following general fact. 
   If the varieties generated by classes $\clC_1$ and $\clC_2$ are locally finite, then the 
   variety generated by  the class  $\clC_1 \cup \clC_2$ is locally finite as well:  $\clC_1 \cup \clC_2$ is uniformly locally finite by Malcev criterion 
   given in Theorem \ref{Malcev73}.}   
   %\cite[Section 14, Theorem 3]{Malcev73}.} 
   Then $L$ is locally tabular by Lemma~\ref{lem:quotient-uniformly-tunable}.

\end{remark} 
\ISLater{Words that this can be done for $\LS{5}\times \LS{5}$}

